Mathemyths: Leveraging Large Language Models to Teach Mathematical Language through Child-AI Co-Creative Storytelling

Mathematical language is a cornerstone of a child's mathematical development, and children can effectively acquire this language through storytelling with a knowledgeable and engaging partner. In this study, we leverage the recent advances in large language models to conduct free-form, creative conversations with children. Consequently, we developed Mathemyths, a joint storytelling agent that takes turns co-creating stories with children while integrating mathematical terms into the evolving narrative. This paper details our development process, illustrating how prompt-engineering can optimize LLMs for educational contexts. Through a user study involving 35 children aged 4-8 years, our results suggest that when children interacted with Mathemyths, their learning of mathematical language was comparable to those who co-created stories with a human partner. However, we observed differences in how children engaged with co-creation partners of different natures. Overall, we believe that LLM applications, like Mathemyths, offer children a unique conversational experience pertaining to focused learning objectives.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> sections/1-introduction.tex <==
\section{Introduction}
Math is a fundamental building block in children's early education and is a strong predictor of their future achievements~\cite{bynnerDoesNumeracyMatter1997,duncanSchoolReadinessLater2007,parsonsDoesNumeracyMatter2005a,saramaEarlyChildhoodMathematics2009,starkeyEnhancingYoungChildren2004}. 
Particularly in early childhood, mathematical learning is not just about learning to count or calculate; it also emphasizes the ability to understand and apply mathematical language, such as ``half'' or ``equal''. Children often learn these words through everyday conversations with others~\cite{thippana2020parents}. For instance, when a parent asks, ``Do you have more cookies than me?'' they are introducing the quantitative term ``more.'' However, studies have found that the amount of math language children encounter to through these everyday, spontaneous conversations can vary greatly, which often aligns with socioeconomic differences. This variation may have translated into disparities in early math abilities ~\cite{elliott2018ses}. 

To enrich children experience of math language beyond everyday conversations, researchers have emphasized the importance of including a \textit{language} component in general mathematics instruction, which allows children to engage with math language in a more systematic way. However, it is challenging to teach math language abstractly to young children. One of approaches widely used with preschool and early elementary school children is to embed math language within the context of \textit{narrative stories}, making abstract language more tangible and engaging for young learners \cite{purpuraCausalConnectionsMathematical2017,hassinger-dasReadingStoriesLearn2015}. This type of story-based learning typically involves encouraging children to participate in dialogues about the storylines and key math terms, guided by a more knowledgeable individual, be it a parent, teacher, or older peer ~\cite{purpuraCausalConnectionsMathematical2017,hassinger-dasReadingStoriesLearn2015,busJointBookReading1995,durantiRethinkingContextLanguage1992a,morrowRetellingStoriesStrategy1985}. Yet, the practicality of teaching math language through joint storytelling is debatable, as it demands a one-on-one engaged storytelling session that is logistically infeasible given the limited resources most educational institutions face ~\cite{purpuraDevelopmentMathematicalLanguage2019,purpuraCausalConnectionsMathematical2017,purpuraEngagingCaregiversChildren2021}. 

In response to this challenge, researchers have long been investigating AI's potential to simulate human-like storytelling interactions~\cite{chungTaleBrushSketchingStories2022,osoneBunChoAISupported2021a,leeInteractiveChildrenStory2022,osoneBunChoAISupported2021a,yuanWordcraftStoryWriting2022,shakeriSAGACollaborativeStorytelling2021}. 
However, before the emergence of Large Language Models (LLMs), AI was primarily optimized for structured interactions with children, such as asking questions and providing evaluative feedback~\cite{ruanSupportingChildrenMath2020, xuElinorTalkingMe2022}. 
It is with the recent advancements in LLMs, notably GPT-4~\cite{GPT4}, that the technical difficulty of facilitating spontaneous and creative conversations has started to see promising developments~\cite{kasneciChatGPTGoodOpportunities2023}. 
However, the feasibility and efficacy of utilizing LLMs as co-creators in children's storytelling for learning mathematical language remains unclear. Moreover, from a product development perspective, it is unclear what specific workflow is necessary to tailor LLMs' capacities to a younger audience ~\cite{weiEmergentAbilitiesLarge2022}.

This study outlines the development process for creating \textsc{Mathemyths}\footnote{Source code: \url{https://github.com/anonymous-for-blind-review}}, a novel co-creative storytelling system powered by a GPT-based conversational agent, aiming at teaching mathematical language to children (Figure~\ref{teaser_figure}). We then present empirical findings from a user study comparing learning outcomes using \textsc{Mathemyths} to those of a comparable human-based interaction. Specifically, we aim to answer the following three research questions: 

\begin{enumerate}
  \item[\textit{\textbf{RQ1}}] \textit{How can prompt engineering be employed to optimize LLMs as story co-creators tailored for children's educational purposes?}
  \item[\textit{\textbf{RQ2}}] \textit{Do interactions with LLMs effectively engage children and provide an enjoyable experience during the co-creation of stories?}
  \item[\textit{\textbf{RQ3}}] \textit{Can children's such interactions with LLMs result in comparable learning outcomes seen in human-child storytelling interactions?}
\end{enumerate}

Our results indicate that when children interacted with \textsc{Mathemyths}, their learning of mathematical language appeared to be comparable to those who co-created stories with a human partner. However, we observed differences in how children engage with co-creation partners of different natures. Specifically, the stories co-created by children and AI tended to be more math-focused and matter-of-fact, while those co-created by children and human partners were more narratively rich. While it is beyond the scope of this study to determine which story co-creation patterns are most educationally beneficial, we believe that LLM applications, such as \TOOL, can offer children a unique conversational experience, complementing their interactions with others. Overall, our findings suggest that LLMs can be engineered to create applications that support children's learning. Additionally, they highlight areas where further considerations are needed to ensure the technology is both supportive and effective for diverse learning experiences. 

\looseness=-1



%(for example, saying ``\textit{take away two apples from the basket with five apple}s''), many find it challenging to transition from this informal, everyday language into formalized, academic language (``\textit{subtract 2 from 5}''). Such academic language is crucial for disciplinary learning in mathematics ~\cite{schleppegrellLinguisticChallengesMathematics2007}.\looseness=-1



==> sections/2-related-work-2.tex <==
\section{Related Work}
In this section, we review research on (1) teaching math language through interactive storytelling, (2) conversational interfaces for children, and (3) large language models in Human-Computer Interaction (HCI).

\subsection{Teaching Math Language through Interactive Storytelling}

% \subsubsection{Early Mathematics Education}

Children's mathematical abilities are significantly influenced by their language skills~\cite{morrowRetellingStoriesStrategy1985, parsonsDoesNumeracyMatter2005a, sunCollaborativeStorytellingRobot2017, wongSpokenNarrativeAssessment2016, wuImprovingVocabularyAcquisition2008, xuDialogueConversationalAgent2022,  zhangStoryBuddyHumanAICollaborative2022}. 
Indeed, the Common Core State Standards highlight the need for students to be able to understand and apply specific mathematical language to describe the math concepts ~\cite{akkus2016common}. For instance, by second grade, students are expected to be familiar with terminology associated with fundamental math operations: addition, subtraction, multiplication, and division. Nevertheless, while some of this math language can be replaced by informal, everyday expressions (e.g., ``putting together'' as opposed to ``addition'') to convey a similar meaning, equipping students with precise math terminologies is still necessary. Such terminology serves as a bridge to help children transition from their concrete everyday way of thinking to more abstract analytical thinking.

Math discourse or "math talk", which is conversations around math concepts, is a powerful mechanism to support children's development of mathematical language. This approach is especially effective when interactions are coupled with constructive feedback ~\cite{KIEMER201594} and diverse question types designed to drive the conversation based on children's interests ~\cite{MercerneillLittletonkaren2007}. Additionally, explicit math language teaching – making the language transparent in its meaning ~\cite{Adler1998ALO}, is crucial during these dialogic exchanges. While actively listening to and validating learners' viewpoints, it is advisable for teachers to provide support through clear instructions and explanations~\cite{Adler1998ALO} to help students decipher the intricacies of technical language and clarify relationships ~\cite{schleppegrell2007linguistic}. For young children who have not started formal school yet, such math talk can be grounded in everyday problems (e.g., who has the most apples) or a narrative plotline. 


%Thus, challenges in language and math often co-occur, especially among low SES children, highlighting the need for concurrent language and math education~\cite{lewisPrevalenceSpecificArithmetic1994,mannkoepkeIntersectionMathReading2013,hanichPerformanceDifferentAreas2001,jordanMathematicalThinkingSecondGrade2000,jordanAssessingEarlyArithmetic1994,jordanSocioeconomicVariationNumber2009,starkeyEnhancingYoungChildren2004,pungelloEffectsSocioeconomicStatus2009}.
%While general language skills may not directly benefit mathematical knowledge, recent research highlights the role of mathematical language~\cite{kungRoleMathematicalLanguage2019,purpuraCausalConnectionsMathematical2017,sonParentalMathTalk2020}, \ie the key words and concepts (e.g., \textit{add}, \textit{subtract}, \textit{divide}, \textit{multiply}) that are required for math talk~\cite{hanChineseEnglishMathematics2001}.
% Studies show that a child's grasp of mathematical language correlates positively with their mathematical abilities~\cite{kungRoleMathematicalLanguage2019,purpuraNonlinearRelationsApproximate2015}.  
%Notably, Researchers like Purpura and Logan~\cite{purpuraNonlinearRelationsApproximate2015} found that understanding mathematical terms improves subsequent mathematical performance~\cite{kungRoleMathematicalLanguage2019,purpuraNonlinearRelationsApproximate2015}, establishing a causal relationship between mathematical language and mathematical abilities~\cite{purpuraCausalConnectionsMathematical2017}.
%Hence, the importance of teaching mathematical language is evident.\looseness=-1

Based on this, a number of interventions have been proposed to enhance children's mathematical language using a storytelling approach ~\cite{glaserNarrativebasedLearningPossible2009,hassinger-dasReadingStoriesLearn2015a,hojnoskiEmbeddingMathematicalDialogue2014,jenningsIncreasingInterestAchievement1992a,powellInfluenceMathematicsVocabulary2015}.
For example, Purpura et al.~\cite{purpuraCausalConnectionsMathematical2017}demonstrated the effectiveness of a dialogic storybook reading program that incorporated question-answer exchanges to encourage verbal responses and higher-order thinking in children. In this program, the researchers also explicitly defined and explained mathematical language terminology, resulting in improvements in both mathematical language skills and mathematical knowledge.   
Furthermore, researchers have suggested that instead of merely having dialogues around existing stories, involving children in the story creation process can be valuable. However, children often struggle to generate stories independently due to their still developing language skills. Thus, it is important to pose questions to guide children's responses or offer constructive feedback responsive to children's contributions. Such \textit{question-feedback-scaffolding} could potentially lower the cognitive demand required for certain challenges children face when continuing the story. 

Overall, past literature suggests situating and defining mathematical terminology in a narrative co-created by children and their partners effectively enhances children's mathematical knowledge and skills. This lays the groundwork for our research, which employs LLMs to emulate this approach.
%which can easily lead to exhaustion of available materials, potentially causing children to feel disinterested after repeated readings~\cite{biemillerEffectiveMethodBuilding2006}.
%It also requires skilled interventionists to restrictively follow a given routine and employ standard strategies like how to ask questions~\cite{purpuraCausalConnectionsMathematical2017}, making it less accessible to most children and families, especially those of low SES.
%Thus, a new accessible, diverse, and interactive intervention mechanism is needed.\looseness=-1

%Beyond math education in narrative-based learning, a body of research underscores the significance of children's active involvement in story creation processes~\cite{ainaImportanceOralStorytelling1999,schiroOralStorytellingTeaching2004,calkinsChildrenRewritingStrategies1980}, 
% such as oral storytelling~\cite{ainaImportanceOralStorytelling1999,schiroOralStorytellingTeaching2004} and story writing or rewriting~\cite{calkinsChildrenRewritingStrategies1980}), 
%rather than being solely passive readers or listeners. 
%This active engagement in creative storytelling has been shown to expand vocabulary~\cite{ainaImportanceOralStorytelling1999}, improve narrative comprehension~\cite{sunCollaborativeStorytellingRobot2017}, and hasten cognitive development~\cite{durantiRethinkingContextLanguage1992}.
%Joint storytelling, a common creative activity often involving interventionists and children co-constructing narratives~\cite{koenigkellasFindingMeaningDifficult2006,treesTellingTalesEnacting2009}, exemplifies such engagement.
%It offers children an opportunity to use language to express concrete meaning~\cite{durantiRethinkingContextLanguage1992}, facilitating early literacy acquisition~\cite{zivanParentChildJoint2020}.
% During conversational storytelling, it is essential to ensure that children actively participate, rather than merely listen passively~\cite{morganDialogicReadingPotential2008}.
%Therefore, joint storytelling could be potentially efficient in teaching mathematical language.

%Moreover, previous research has suggested several efficacious communication strategies for adults to motivate and inspire children in this process.
%One prevalent method is the \textit{question-feedback-scaffolding} framework~\cite{xuElinorTalkingMe2022}.
%First, asking children questions stimulates their thoughtful responses. 
%Second, offering positive feedback acknowledges their contributions. 
%Third, providing scaffolding inspires children's creativity if they struggle to continue the story.
%Xu et al.~\cite{xuElinorTalkingMe2022} demonstrated the effectiveness of this framework in engaging children and enhancing their scientific learning.
%Thus, in our research, we apply this question-feedback-scaffolding framework to efficiently guide children throughout the child-AI joint storytelling process.\looseness=-1

\subsection{Conversational Interfaces for Children}

With the rapid advancement of AI, conversational user interfaces (CUIs) now simulate speech-based, interpersonal interactions with children~\cite{porcheronVoiceInterfacesEveryday2018}.
These interactions remove the literacy barriers of many graphic user interfaces (GUIs), releasing the screen tensions between children and their parents~\cite{hinikerScreenTimeTantrums2016,kawasWhenScreenTime2021a}.
Previous research has identified two prevalent types of interactions that children tend to have with CUIs~\cite{xuAreCurrentVoice2021}: smart speakers supporting open-domain conversations (e.g., Apple Siri, Amazon Alexa, Google Assistant) and voice-based apps with agent-led context-specific conversations~\cite{leeDAPIEInteractiveStepbyStep2023,beneteauParentingAlexaExploring2020a,bentleyUnderstandingLongtermUse2018,lovatoHeyGoogleUnicorns2019,lovatoYoungChildrenVoice2019}.
Voice-based apps are recognized as accessible technologies for low-SES families since they can be easily integrated into commonplace devices (\eg mobile phones, laptops, computers) without relying on costly external devices such as robots~\cite{dietzStoryCoderTeachingComputational2021,madaioCollectiveSupportIndependent2020}.
Our system is one such accessible voice-based app devoid of any GUIs, featuring a conversational agent specifically designed for children's mathematical language learning and joint storytelling.\looseness=-1

Notably, CUIs-based apps present an encouraging modality for educating young children in numerous disciplines, including scientific learning~\cite{xuElinorTalkingMe2022}, computational thinking~\cite{dietzStoryCoderTeachingComputational2021}, and literacy development~\cite{xuAreCurrentVoice2021}.
Specifically, researchers posit that these CUIs could significantly contribute to children's language development by acting as language partners~\cite{xuExploringYoungChildren2020,bieleHowMightVoice2019}.
Few efforts aim at fostering children's mathematical language development through  CUIs~\cite{hoDesigningParentchildrobotInteractions2023,xuMathKingdomTeachingChildren2023b}.
They either designed a voice-guided game~\cite{xuMathKingdomTeachingChildren2023b} or a social robot~\cite{hoDesigningParentchildrobotInteractions2023} to facilitate math talk between children and parents.
Although these efforts overlook co-creative storytelling as an effective method, they provide us with valuable insights on taking a voice-based interaction to initiate mathematical communication with children and resolve the issue of low engagement~\cite{hoDesigningParentchildrobotInteractions2023,xuMathKingdomTeachingChildren2023b}.\looseness=-1

Furthermore, HCI scholars have developed an extensive array of CUIs to enhance various facets of storytelling for children~\cite{zhangStoryDrawerChildAI2022,zhangStoryDrawerCoCreativeAgent2021,xuDialogueConversationalAgent2022,xuExploringYoungChildren2020,wuImprovingVocabularyAcquisition2008}.
Some of these agents are specifically tailored for joint storytelling~\cite{sunCollaborativeStorytellingRobot2017,ligthartDesignPatternsInteractive2020}.
The prevailing model involves the agent listening to a child's story and subsequently sharing one in return~\cite{bersInteractiveStorytellingSystems1998,ryokaiVirtualPeersPartners2003,westlundInterplayRobotLanguage2015}.
For instance, the SAGE system~\cite{bersInteractiveStorytellingSystems1998} begins by listening to a child's story, subsequently responding with a traditional tale, typically imparting wisdom.
However, such interactions often appear rigid as the agent contributes minimally during the child's story, instead waiting for the child to conclude before offering its narrative.
To advance beyond this limitation, Sun et al.~\cite{sunCollaborativeStorytellingRobot2017} enabled the computational agent to introduce new characters and objects during the children's storytelling sessions.
In a similar vein, Ligthart et al.~\cite{ligthartDesignPatternsInteractive2020} facilitated children in shaping the storyline by making decisions regarding the characters' actions within the agent's narrative.
Yet, these efforts either employ a Wizard-of-Oz setup, with experimenters substituting the agent~\cite{sunCollaborativeStorytellingRobot2017}, or adhere strictly to a predefined multi-branch narrative structure~\cite{ligthartDesignPatternsInteractive2020}.
Both techniques attempt to enhance children's autonomy, but neither provides a realistic and flexible joint storytelling experience.\looseness=-1

A study by Xu et al.~\cite{xuAreCurrentVoice2021} discovered that most CUIs are incapable of conducting open-ended dialogues and providing prolonged interactive opportunities, thus inhibiting their potential to stimulate children's language output and enrich children's language exposure. 
They rely on ``pseudo-conversation'', where the agent adheres to pre-determined dialogue flows when interacting with children~\cite{xuAreCurrentVoice2021}.
Evidently, such a pre-determined paradigm is not suitable for creative activities like joint storytelling, given that children may produce a variety of creative responses. 
The agents must be adaptable and flexible to incorporate children's responses into their feedback.
Hence, our paper attempts to implement ``true conversion''---defined as multiple parties ``mutually orienting to, and collaborating in order to achieve, orderly and meaningful communication''~\cite{enyiLanguageInteractionalDiscourse2015}---in CUIs-based apps.\looseness=-1

\subsection{Large Language Models}

Pre-trained large language models (LLMs), such as GPT-3~\cite{brownLanguageModelsAre2020a} and GPT-4~\cite{GPT4}, have significantly advanced natural language processing (NLP) in recent years. 
These models, trained on colossal amounts of text data, can generalize to downstream tasks like text generation~\cite{weiEmergentAbilitiesLarge2022}. 
One key capability derived from the large model size is \textit{prompting}~\cite{weiEmergentAbilitiesLarge2022}, which allows individuals to provide specific textual instructions and examples~\cite{zamfirescu-pereiraWhyJohnnyCan2023} to guide the model's task execution. 
Although prompting LLMs may not consistently surpass benchmark models, it offers a lightweight approach to achieve competitive performance across a variety of tasks~\cite{chowdheryPaLMScalingLanguage2022,brownLanguageModelsAre2020a}. 
The concept of prompting LLMs remains a compelling research topic within the HCI community. 
Our work extends previous research by introducing a set of prompting techniques iteratively designed to optimize LLMs as story co-creators tailored for children’s educational purposes.\looseness=-1

CUIs powered by LLMs, such as ChatGPT~\cite{IntroducingChatGPT}, have demonstrated their prowess in facilitating responsive and engaging dialogues. 
Unlike traditional CUIs, they are not constrained by a pre-determined dialogue paradigm or reliant on pre-written responses.
One of their standout features is the ability to generate contextually relevant and coherent responses based on the input they receive so far~\cite{weiEmergentAbilitiesLarge2022}. 
% This capability makes them especially suited for open-ended interactions with children, providing a more genuine conversational experience~\cite{leeDAPIEInteractiveStepbyStep2023}.
% Furthermore, with the vast amount of training data at their disposal, these models excel at producing diverse and contextually appropriate responses according to the prompts. 
This capability positions them to achieve ``true conversation'', wherein they can effectively collaborate with children, ensuring a more natural and enriching dialogue~\cite{leeDAPIEInteractiveStepbyStep2023}.
Thus, this paper harnesses the adaptability and flexibility of LLMs, aiming to forge a dynamic and collaborative storytelling experience for children, thereby fostering their math language growth and stimulating their creative expression.

Recently, numerous researchers have endeavored to incorporate LLMs into educational technologies~\cite{kasneciChatGPTGoodOpportunities2023}. 
These adaptations have seen the utilization of LLMs in creating educational content~\cite{dijkstraReadingComprehensionQuiz2022a,gabajiwalaQuizMakerAutomatic2022a}, enhancing student engagement and interaction~\cite{baoCanHomeUse2019,taiImpactGoogleAssistant2020,abdelghaniGPT3drivenPedagogicalAgents2023}, and personalizing learning experiences~\cite{sailerAdaptiveFeedbackArtificial2023}. 
For instance, LLMs have been used to generate children's narratives~\cite{guanKnowledgeEnhancedPretrainingModel2020,alabdulkarimAutomaticStoryGeneration2021}, some of which have even been sold publicly~\cite{messickChatGPTAuthor1002023}. 
In a different research trajectory, several scholars have used LLMs to create intelligent learning partners capable of collaborating with humans~\cite{jiSystematicReviewConversational2022}, providing feedback~\cite{jiaAllinoneMultitaskLearning2021} and encouraging students~\cite{elshazlyEffectsArtificialIntelligence2021,taiImpactGoogleAssistant2020}. 
One common application involves employing LLMs as a conversational partner in written or oral form, such as in the context of task-oriented dialogues that offer language practice opportunities~\cite{elshazlyEffectsArtificialIntelligence2021}.
Building on these advancements in LLMs, our work aims to apply LLMs in CUIs to enable child-AI collaborative storytelling for mathematical language learning.\looseness=-1



==> sections/2-related-work.tex <==
\section{Related Work}
In this section, we review research on (1) mathematical language, (2) interactive storytelling for children, (3) educational technologies with LLMs, and (4) voice interfaces for children in Human-Computer Interaction (HCI).

% \subsection{Early Mathematics Education}

\subsection{Mathematical Language}

% \subsubsection{Early Mathematics Education}


The development of early mathematical knowledge, which begins before school entry, is critical to later mathematical abilities~\cite{gerstenEarlyIdentificationInterventions2005,saramaEarlyChildhoodMathematics2009,starkeyEnhancingYoungChildren2004}, academic success~\cite{bynnerDoesNumeracyMatter1997,duncanSchoolReadinessLater2007,parsonsDoesNumeracyMatter2005a}, health and personal well-being~\cite{parsonsDoesNumeracyMatter2005a}, SES levels, and STEM (Science, Technology, Engineering, and Mathematics) career potential~\cite{waiSpatialAbilitySTEM2009}. 
% The development of early mathematical knowledge, which begins before school entry, is critical to the development of later mathematics skills~\cite{gerstenEarlyIdentificationInterventions2005,saramaEarlyChildhoodMathematics2009,starkeyEnhancingYoungChildren2004} and academic and life outcomes~\cite{bynnerDoesNumeracyMatter1997,duncanSchoolReadinessLater2007,parsonsDoesNumeracyMatter2005a}, including entry into STEM (Science, Technology, Engineering, and Mathematics) fields~\cite{waiSpatialAbilitySTEM2009}, socioeconomic status (SES) levels, as well as health and personal well-being~\cite{parsonsDoesNumeracyMatter2005a}.
Of note, mathematical abilities vary widely among children, with language skills being a significant contributing factor~\cite{lefevrePathwaysMathematicsLongitudinal2010,pengExaminingMutualRelations2020,purpuraEarlyLiteracyEarly2011}.

Existing research demonstrates a strong interplay between mathematical and language skills in children's academic development~\cite{jenningsIncreasingInterestAchievement1992,hooperLongitudinalPredictorsReading2010,purpuraEarlyLiteracyEarly2011a,romanoSchoolReadinessLater2010,miuraLanguageSupportsMathematics2013}. 
These language skills, such as vocabulary, refine children's quantitative understanding~\cite{spelkeWhatMakesUs2003}, and aid in mathematical communication~\cite{chardPreventingEarlyMathematics2008,clementsEarlyChildhoodMathematics2011,schleppegrellLinguisticChallengesMathematics2007}, influencing their logical and mathematical cognitive development~\cite{houdeNeuralFoundationsLogical2003}.
% There is a long tradition of research that investigates the relationship between mathematics and language in children's academic development~\cite{jenningsIncreasingInterestAchievement1992,hooperLongitudinalPredictorsReading2010,purpuraEarlyLiteracyEarly2011a,romanoSchoolReadinessLater2010}. 
% Language skills (\eg vocabulary, oracy, reading, listening) are presumed to support mathematical development~\cite{miuraLanguageSupportsMathematics2013} as children utilize language skills to refine their quantitative understanding~\cite{spelkeWhatMakesUs2003}. 
% At the same time, successful mathematical curriculum relies on effective mathematical communication~\cite{chardPreventingEarlyMathematics2008,clementsEarlyChildhoodMathematics2011,schleppegrellLinguisticChallengesMathematics2007}, which positively affects children's logical and mathematical cognitive development~\cite{houdeNeuralFoundationsLogical2003}.
Interestingly, difficulties in mathematics and difficulties in literacy and language often co-occur~\cite{lewisPrevalenceSpecificArithmetic1994,mannkoepkeIntersectionMathReading2013}.
Children facing difficulties in both language and math tend to perform worse in math compared to those with only math difficulties~\cite{hanichPerformanceDifferentAreas2001,jordanMathematicalThinkingSecondGrade2000}.
% Children who experience difficulties in both mathematics and language tend to have poorer mathematical knowledge than children who have difficulties in mathematics alone~\cite{hanichPerformanceDifferentAreas2001,jordanMathematicalThinkingSecondGrade2000}. 
Regrettably, low SES children often exhibit deficits in both areas~\cite{jordanAssessingEarlyArithmetic1994,jordanSocioeconomicVariationNumber2009,starkeyEnhancingYoungChildren2004,pungelloEffectsSocioeconomicStatus2009}, emphasizing the importance of simultaneously teaching language and mathematical skills.
% Unfortunately, children from low SES families often have deficits in both mathematics~\cite{jordanAssessingEarlyArithmetic1994,jordanSocioeconomicVariationNumber2009,starkeyEnhancingYoungChildren2004} and language skills~\cite{pungelloEffectsSocioeconomicStatus2009}. 
% Language deficits are thought to be one explanation for SES-based differences in mathematics performance~\cite{jordanAssessingEarlyArithmetic1994a,jordanSocioeconomicVariationNumber2009,starkeyEnhancingYoungChildren2004}. 
% Therefore, it is important to training children language skills and teaching their mathematics simultaneously.

However, improving children's general language skills seems not directly benefit their mathematics knowledge~\cite{jordanBuildingKindergartnersNumber2012}.
It remains to be determined which aspects of language boost mathematical learning.
% A likely explanation for this lack of improvement is that the language targeted through a general language intervention includes different words than those utilized in mathematical instruction (\ie mathematical language)~\cite{harmonResearchVocabularyInstruction2005}.
Recent research highlights the role of mathematical language~\cite{kungRoleMathematicalLanguage2019,purpuraCausalConnectionsMathematical2017,sonParentalMathTalk2020}, \ie the key words and concepts (e.g., \textit{add}, \textit{subtract}, \textit{divide}, \textit{multiply}) that are required for math talk~\cite{hanChineseEnglishMathematics2001}.
% A recent line of research emphasizes the role of mathematical language in children's mathematical abilities~\cite{kungRoleMathematicalLanguage2019,purpuraCausalConnectionsMathematical2017,sonParentalMathTalk2020}.
% There is two different definitions of mathematical language~\cite{turanMathematicalLanguageMathematical2022}: one is restricted to quantitative (\eg \textit{more}, \textit{fewest}, \textit{a little bit}) and/or spatial (\eg \textit{before}, \textit{after}, \textit{nearest}) terms~\cite{purpuraCausalConnectionsMathematical2017}; another is more broad to include children's understanding of mathematical concepts such as words related to counting and calculating~\cite{klibanoffPreschoolChildrenMathematical2006}.
Studies show that a child's grasp of mathematical language correlates positively with their mathematical abilities~\cite{kungRoleMathematicalLanguage2019,purpuraNonlinearRelationsApproximate2015}. 
% Already in preschool, young children's understanding of mathematical language positively correlates with their mathematical abilities~\cite{kungRoleMathematicalLanguage2019,purpuraNonlinearRelationsApproximate2015}. 
Notably, Purpura and Logan~\cite{purpuraNonlinearRelationsApproximate2015} found that understanding mathematical terms improves subsequent mathematical performance, establishing a causal relationship between mathematical language and mathematical abilities~\cite{purpuraCausalConnectionsMathematical2017}.
% For example, Purpura and Logan~\cite{purpuraNonlinearRelationsApproximate2015} observed that children who are good at understanding mathematical terms performed better on subsequent tests of mathematical ability.
% In their following studies, Purpura and colleagues further found the causal relationship between mathematical language and children's mathematical abilities~\cite{purpuraCausalConnectionsMathematical2017}.
Hence, the importance of teaching mathematical language is evident.
% \hl{In this paper, we focus on the restrictive definition of mathematical language, considering its suitability for young children, as it requires no explicit mathematical knowledge or precise quantitative skills. 
% Further, given the extensive range of quantitative and spatial terms, we primarily use quantitative terms to demonstrate our system.}
% In this paper, we set mathematical language as the restrictive definition since it requires no mathematical knowledge or exact quantitative skills, which is more suitable for children at a young age.
% Specifically, we take quantitative terms as examples to demonstrate our system as the complete vocabulary of quantitative and spatial terms is too many to cover at one time.

A few interventions have been proposed to enhance children's mathematical language, with a predominant focus on storytelling activities such as storybook reading~\cite{hassinger-dasReadingStoriesLearn2015a,hojnoskiEmbeddingMathematicalDialogue2014,jenningsIncreasingInterestAchievement1992a,powellInfluenceMathematicsVocabulary2015}.
Among those, Clements et al.~\cite{clementsBackgroundResearchEarly2013} underlined the value of interaction in storytelling-based methods.
% There is a few interventions to improve mathematical language~\cite{hassinger-dasReadingStoriesLearn2015a,hojnoskiEmbeddingMathematicalDialogue2014,jenningsIncreasingInterestAchievement1992a,powellInfluenceMathematicsVocabulary2015}, mainly focusing on story reading or parent-child shared book reading.
% Among those, Clements et al.~\cite{clementsBackgroundResearchEarly2013} postulated that interactions rich in mathematical language interventions are important in developing children's early mathematical knowledge.
In response, Purpura et al.~\cite{purpuraCausalConnectionsMathematical2017} proposed a dialogic reading storybook intervention incorporating question-answer exchanges to eliciting verbal responses and descriptions from children.
The results demonstrated such a storytelling-based method not only improved children's mathematical language, but increased their overall mathematics abilities as well. 
However, this method, though effective, is resource-intensive and relies on predefined storybooks and planned questions~\cite{purpuraDevelopmentMathematicalLanguage2019,purpuraEngagingCaregiversChildren2021}, which can easily lead to exhaustion of available materials, potentially causing children to feel disinterested after repeated readings~\cite{biemillerEffectiveMethodBuilding2006}.
It also requires skilled human facilitators to restrictively follow a given routine and employ standard strategies like how to ask questions~\cite{purpuraCausalConnectionsMathematical2017}, making it less accessible to most children and families, especially those of low SES.
Therefore, a new accessible, diverse, and interactive intervention mechanism is needed.
% Therefore, it is important to invent a new interactive intervention mechanism which is easy to access and can diversify its content to engage children.

In HCI, technology-based scaffolding for early math learning has been explored through augmented reality, educational games, and embodied interaction~\cite{besevliMaRTDesigningProjectionbased2019,kangARMathAugmentingEveryday2020,liExploringTangibleInteraction2019,vanderstappenMathBuilderCollaborativeAR2019,abrahamsonEmbodiedinteractionDesignFramework2011,ruanSupportingChildrenMath2020}.
% In the field of Human-Computer Interaction (HCI), there is many attempts to scaffold children's early mathematical learning through technology such as augmented reality, educational games, and embodied interaction~\cite{besevliMaRTDesigningProjectionbased2019,kangARMathAugmentingEveryday2020,liExploringTangibleInteraction2019,vanderstappenMathBuilderCollaborativeAR2019,abrahamsonEmbodiedinteractionDesignFramework2011,ruanSupportingChildrenMath2020}.
Only a few efforts aim at children's mathematical language development~\cite{hoDesigningParentchildrobotInteractions2023,xuMathKingdomTeachingChildren2023b}.
They either designed a voice-guided game~\cite{xuMathKingdomTeachingChildren2023b} or a social robot~\cite{hoDesigningParentchildrobotInteractions2023} to facilitate math talk between children and their parents.
They provide us with valuable insights on taking a voice-based interaction manner, initiating mathematical communication with children, and resolving the issue of low engagement~\cite{hoDesigningParentchildrobotInteractions2023,xuMathKingdomTeachingChildren2023b}.
However, they both required parental guidance throughout and did not address the issues associated with previous storytelling-based interventions.
% For example, Xu et al.~\cite{xuMathKingdomTeachingChildren2023b} designed a voice-based game that engages children to design their virtual avatars using mathematical descriptions.
% Its need-finding study provides us with valuable insights on taking a voice-based interaction manner, initiating mathematical communication with children, and resolving the issue of low engagement.
% However, this method required parental guidance throughout, negating independent learning~\cite{zhangStoryBuddyHumanAICollaborative2022}, and did not address the issues associated with dialogic reading interventions.
This paper proposes a novel, automated, co-creative storytelling intervention drawn on joint storytelling and large language models, enabling engaging, diverse, and accessible mathematical language learning for children.
% Therefore, in this paper, we draw on the advancements of interactive storytelling systems and large language models to automate a novel co-creative storytelling intervention so that children's mathematical language learning can be implemented independently, diversely, and at scale.

% \subsubsection{The Relations of Language and Mathematics Development}

% \subsubsection{Mathematics-Specific Language}

% \subsubsection{Interventions to Improve Mathematical Language}

% \newpage
\subsection{Interactive Storytelling for Children}

Research has long appreciated narratives as a medium for knowledge dissemination and as instructional materials in educational settings, giving rise to the concept of narrative-based learning~\cite{glaserNarrativebasedLearningPossible2009}.
This approach encourages children to read or listen to stories, fostering the development of mental models for abstract concepts~\cite{schrawSituationalInterestLiterary1997a,glaserNarrativebasedLearningPossible2009} and enhancing self-regulated learning~\cite{perryYoungChildrenSelfregulated1998}.
Importantly, a body of research underscores the significance of children's active involvement in story creation processes such as oral storytelling~\cite{ainaImportanceOralStorytelling1999,schiroOralStorytellingTeaching2004} and story writing or rewriting~\cite{calkinsChildrenRewritingStrategies1980}), rather than being solely passive readers or listeners. 
% For example, they suggested children can orally tell stories~\cite{ainaImportanceOralStorytelling1999,schiroOralStorytellingTeaching2004}, rewrite stories~\cite{calkinsChildrenRewritingStrategies1980}, or waving the story lines through their imagination.
This active engagement in creative storytelling has been shown to expand vocabulary~\cite{ainaImportanceOralStorytelling1999}, increase sentence complexity, improve narrative comprehension~\cite{sunCollaborativeStorytellingRobot2017}, and hasten cognitive development~\cite{durantiRethinkingContextLanguage1992}.

Conversational storytelling, a common creative activity often involving a human partner and children co-constructing narratives~\cite{koenigkellasFindingMeaningDifficult2006,treesTellingTalesEnacting2009}, exemplifies such engagement.
It offers children an opportunity to use language to express concrete meaning~\cite{durantiRethinkingContextLanguage1992}, facilitating early literacy acquisition~\cite{zivanParentChildJoint2020}.
% However, parents and guardians may not always have the time or energy to engage their children in joint storytelling, despite their best intentions~\cite{zhangStoryBuddyHumanAICollaborative2022}. 
During conversational storytelling, it is essential to ensure that children actively participate, rather than merely listen passively~\cite{morganDialogicReadingPotential2008}.
In response, previous research has suggested several efficacious communication strategies for adults to motivate and inspire children.
One prevalent method is the question-feedback-scaffolding framework~\cite{xuElinorTalkingMe2022}.
First, asking children questions stimulates their thoughtful responses. 
Second, offering positive feedback acknowledges their contributions. 
Third, providing scaffolding inspires children's creativity if they struggle to continue the story.
Xu et al. demonstrated the effectiveness of this framework in engaging children and enhancing their scientific learning~\cite{xuElinorTalkingMe2022}.
Thus, in our research, we apply this question-feedback-scaffolding framework to efficiently guide children through the child-AI joint storytelling process.

In recent years, HCI scholars have developed an extensive array of interactive, both virtual and tangible, agents designed to enhance various facets of storytelling for children~\cite{zhangStoryDrawerChildAI2022,zhangStoryDrawerCoCreativeAgent2021,xuDialogueConversationalAgent2022,xuExploringYoungChildren2020,wuImprovingVocabularyAcquisition2008}.
Some of these agents are specifically tailored for joint storytelling~\cite{sunCollaborativeStorytellingRobot2017,ligthartDesignPatternsInteractive2020}.
The prevailing model involves the agent listening to a child's story and subsequently sharing one in return~\cite{bersInteractiveStorytellingSystems1998,ryokaiVirtualPeersPartners2003,westlundInterplayRobotLanguage2015}.
For instance, the SAGE system~\cite{bersInteractiveStorytellingSystems1998} begins by listening to a child's story, subsequently responding with a traditional tale, typically imparting wisdom.
% The Sam system [24] was an embodied storytelling virtual character, who was a peer to preschool children and told stories around a figurine and a toy castle. The child was asked to tell his/her own story after Sam had finished.
% However, traditional storytelling robots or virtual characters interact with children in a rigid and sparse way (e.g., [3, 27]). 
However, such interactions often appear rigid as the agent contributes minimally during the child's story, instead waiting for the child to conclude before offering its narrative.
To advance beyond this limitation, Sun et al.~\cite{sunCollaborativeStorytellingRobot2017} enabled the computational agent to introduce new characters and objects during the children's storytelling sessions.
In a similar vein, Ligthart et al.~\cite{ligthartDesignPatternsInteractive2020} facilitated children in shaping the storyline by making decisions regarding the characters' actions within the agent's narrative.
Yet, these efforts either employ a Wizard-of-Oz setup, with experimenters substituting the agent~\cite{sunCollaborativeStorytellingRobot2017}, or adhere strictly to a predefined multi-branch narrative structure~\cite{ligthartDesignPatternsInteractive2020}.
Both techniques failed to provide a realistic and flexible joint storytelling experience for children.

Recently, several studies have ventured into fostering collaboration between AI partners and children in creative activities such as drawing and problem-solving~\cite{aliDesigningGamesEnabling2021,aliEscapeBotSocial2022,alves-oliveiraBoostingChildrenCreativity2016,alves-oliveiraRoboticsBasedInterventionsChildren2021}.
These studies have highlighted the feasibility of co-creative interactions between children and AI, illustrating the profound impact of AI technologies in stimulating children's creativity and improving their engagement. 
One particularly relevant example is StoryDrawer~\cite{zhangStoryDrawerChildAI2022,zhangStoryDrawerCoCreativeAgent2021}, a platform that utilizes a turn-taking collaborative model, enabling the AI to create illustrations as a child narrates a story.  
Inspired by this concept, our work incorporates the turn-taking strategy into the process of joint oral storytelling.
This allows both the child and the agent to contribute equally and alternately to a unique narrative. 
To differentiate this from traditional joint storytelling, we have termed this approach co-creative storytelling.
Moreover, to pursue a flexible interaction and to ensure children's active participation, the agent in our system offers two novel contributions: (1) its ability to naturally continue the story based on children's additions; and (2) its capacity for flexible creativity support by generating immediate prompts based on the question-feedback-scaffolding framework. 

% \subsubsection{Narrative-based Learning}

% \subsubsection{Technologies for Supporting Storytelling}

% \subsection{Technologies That Simultaneously Support Math Learning and Storytelling}

% \subsubsection{Interactive Storytelling with LLMs}


\subsection{Educational Technologies with LLMs}

Pre-trained large language models (LLMs), such as GPT3~\cite{brownLanguageModelsAre2020a} and ChatGPT~\cite{IntroducingChatGPT}, have significantly advanced natural language processing (NLP) in recent years. 
These models, trained on colossal amounts of text data, can generalize to downstream tasks like text generation, question answering, and intent classification~\cite{weiEmergentAbilitiesLarge2022}. 
One key capability derived from the large model size is \textit{prompting}~\cite{weiEmergentAbilitiesLarge2022}, which allows individuals to provide specific textual instructions and examples~\cite{zamfirescu-pereiraWhyJohnnyCan2023}, referred to as \textit{prompts}, to guide the model's task execution. 
Although prompting LLMs may not consistently surpass benchmark models, it offers a lightweight approach to achieve competitive performance across a variety of tasks~\cite{chowdheryPaLMScalingLanguage2022,brownLanguageModelsAre2020a}. 
The concept of prompting LLMs remains a compelling research topic within the community. 
Our work extends previous research by introducing a set of prompting techniques tailored to adapt LLMs for children's storytelling.

Numerous researchers have endeavored to incorporate LLMs into Educational Technologies~\cite{kasneciChatGPTGoodOpportunities2023}. 
These adaptations have seen the utilization of LLMs in creating educational content~\cite{dijkstraReadingComprehensionQuiz2022a,gabajiwalaQuizMakerAutomatic2022a}, enhancing student engagement and interaction~\cite{baoCanHomeUse2019,taiImpactGoogleAssistant2020,abdelghaniGPT3drivenPedagogicalAgents2023}, and personalizing learning experiences~\cite{sailerAdaptiveFeedbackArtificial2023}. 
For instance, a specific study employed GPT-3 to generate questions for text-based learning materials~\cite{bhatAutomatedGenerationEvaluation2022}. 
This approach considerably alleviates the burden of manual quiz design for educators~\cite{dijkstraReadingComprehensionQuiz2022a}. 
Notably, the questions generated by LLMs received favorable ratings from trained research assistants~\cite{bhatAutomatedGenerationEvaluation2022} and proved beneficial in improving student learning outcomes~\cite{dijkstraReadingComprehensionQuiz2022a,bhatAutomatedGenerationEvaluation2022}.
Moreover, LLMs have been used to generate narratives~\cite{guanKnowledgeEnhancedPretrainingModel2020,alabdulkarimAutomaticStoryGeneration2021}, some of which have even been sold publicly~\cite{messickChatGPTAuthor1002023}. 
In a different research trajectory, several scholars have harnessed LLMs to create intelligent learning partners capable of collaborating with humans~\cite{jiSystematicReviewConversational2022}, providing feedback~\cite{jiaAllinoneMultitaskLearning2021}, and encouraging students~\cite{elshazlyEffectsArtificialIntelligence2021,taiImpactGoogleAssistant2020}. 
One common application involves employing LLMs as a conversational partner in written or oral form, such as in the context of task-oriented dialogues that offer language practice opportunities, including pronunciation~\cite{elshazlyEffectsArtificialIntelligence2021}.
Building on these advancements in LLMs and their emergence in Educational Technologies, our work represents the first contribution of applying LLMs to enable child-AI collaborative storytelling for mathematical language learning.

\subsection{Voice Interfaces for Children}

With the rapid advancement of AI, voice user interfaces (VUIs) now exhibit the capability to simulate speech-based, interpersonal interactions with children~\cite{porcheronVoiceInterfacesEveryday2018}.
These interactions remove the literacy barriers of many graphic user interfaces (GUIs), while releasing the screen tensions between children and their parents~\cite{hinikerScreenTimeTantrums2016,kawasWhenScreenTime2021a}.
% Currently, many children already interact regularly with VUIs (e.g., the smart speakers in their own homes), and 
Previous research has identified two prevalent types of interactions that children tend to have with VUIs~\cite{xuAreCurrentVoice2021}: smart speakers supporting open-domain conversations (e.g., Apple Siri, Amazon Alexa, Google Assistant) and voice-based apps with agent-led context-specific conversations~\cite{leeDAPIEInteractiveStepbyStep2023,beneteauParentingAlexaExploring2020a,bentleyUnderstandingLongtermUse2018,lovatoHeyGoogleUnicorns2019,lovatoYoungChildrenVoice2019}.
Voice-based apps are recognized as accessible technologies for low-SES families since they can be easily integrated into commonplace devices (\eg mobile phones, laptops, computers) without relying on costly external devices such as robots~\cite{dietzStoryCoderTeachingComputational2021,madaioCollectiveSupportIndependent2020}.
Our system is one such accessible voice-based app devoid of any GUIs, featuring a conversational agent specifically designed for children's mathematical language learning and joint storytelling simultaneously.

Notably, voice-based apps present an encouraging modality for educating young children in numerous disciplines, including scientific learning~\cite{xuElinorTalkingMe2022}, computational thinking~\cite{dietzStoryCoderTeachingComputational2021}, and literacy development~\cite{xuAreCurrentVoice2021}
Specifically, researchers posit that these VUIs could significantly contribute to children's language development by acting as language partners~\cite{xuExploringYoungChildren2020,bieleHowMightVoice2019}.
However, a study by Xu et al.~\cite{xuAreCurrentVoice2021} discovered that most VUIs are incapable of conducting open-ended dialogues and providing prolonged interactive opportunities, thus inhibiting their potential to stimulate children's language output and enrich children's language exposure. 
They rely on what is termed as ``pseudo-conversation'', where the agent adheres to pre-determined dialogue flows when interacting with children~\cite{xuAreCurrentVoice2021}.
Evidently, such a pre-determined paradigm is not suitable for creative activities like joint storytelling, given that children may produce a variety of creative responses. 
The agents must be adaptable and flexible to incorporate children's responses into their feedback.
Our paper represents the first attempt to implement ``true conversion''---defined as multiple parties ``mutually orienting to, and collaborating in order to achieve, orderly and meaningful communication''~\cite{enyiLanguageInteractionalDiscourse2015}---in voice-based apps.

% \subsection{Collaboration between Child and AI}



==> sections/3-system-design.tex <==
\section{The Development Process of \textsc{Mathemyths}}
Given the strong evidence that children develop math language through storytelling, and considering the unique capabilities of LLMs, we embarked on a design process to conceptualize \TOOL. Our aim was to create a co-creative storytelling system tailored for children aged 4-8, introducing them to mathematical language through voice-based interactions. This initiative served as a case study to explore the potential of LLMs as educational partners for children.\looseness=-1

At its core, \TOOL is designed to collaboratively engage in storytelling by alternating turns with the child. The role of \TOOL within this dynamic is twofold: generating prompts to elicit narrative contributions from the children and continuing the story by utilizing mathematical language based on the children's input. The interaction flow is presented in Fig. ~\ref{fig:all_in_one}. 
The example conversation between a child and \TOOL can be found in Appendix~\ref{sec:example_conversation}.

Given that using LLMs, particularly through prompt engineering, to develop educational tools is a relatively new domain, our design process began by following principles from existing literature. We then engaged in a series of experiments to optimize \TOOL's capabilities for math-focused dialogue. In the remainder of this section, we outline 1) our overall design principles for \TOOL, 2) our method to prompt engineer LLM to serve as the story co-creator, 3) our process to evaluate the prompt-engineered LLM's performance, and 4) the implementation of the \TOOL system. 

\subsection{Design Principles}
Drawing from the literature reviewed above, we incorporated two key design principles into the story co-creation interaction.
 
First, the conversation experience is designed to emulate a joint storytelling activity while the AI partner guides children in this process through a question-feedback-scaffolding framework~\cite{xuElinorTalkingMe2022}. Under this framework, \TOOL initiates the interaction with children by crafting an initial story plot based on children's input about key elements such as the protagonist and setting. It then poses open-ended questions to solicit how children wish the story should progress, such as ``\textit{What will Lucy and Nick do next to make sure they take an equal number of steps to reach the treasure?}'' \TOOL then continues the narrative in line with the children's contributions. In the cases when children require additional support to generate a concrete idea to advance the narratives, \TOOL asked follow-up questions that encourage children to elaborate on or provided suggestions for children to consider (e.g., ``\textit{Do you think Lucy and Nick can take turns counting their steps?}''). The story narratives follow the quest archetype, commonly found in children's literature~\cite{huckChildrenLiteratureElementary2003}, which revolves around a protagonist's pursuit of a specific location, object, or objective, overcoming numerous challenges in the process. 

Second, situated within the narrative structure, \TOOL is also designed to teach math language through exposure (i.e., using math terms in the plots generated by \TOOL) and practice (i.e., posing questions to encourage children to use math terms to continue the stories). In addition, every time \TOOL introduces a math term, it provides an explanation embedded within the narrative context. Given our focus on children aged from four to eight years, the system aimed to focus on six mathematical terms (\textit{sum}, \textit{estimate}, \textit{add}, \textit{subtract}, \textit{equal}, and \textit{half}) frequently found in state and national mathematical knowledge standards for the target age range \cite{councilofchiefstateschoolofficersCommonCoreState2010}. We piloted several other terms (i.e. divide, more, fewer) but ultimately decided on these six as the most appropriate for our chosen age range. Children heard these terms used at least twice per story and defined at least once per story. 




%The question-feedback-scaffolding framework provided children with a structure for story co-creation. The agent initiates the interaction by introducing itself as "Alexa" and asking what the child's name is. This is intended to put the child at ease as it is a social exchange they are used to and is a question they can answer confidently. Alexa also asks about how the child is feeling, which provides an easy entry point to introduce the storytelling game as a way to improve the child's day regardless of how they are feeling. At the beginning of each story, we ensured the agent promoted children's active involvement in story creation processes by soliciting their input for key narrative elements like deciding on the protagonist and setting ~\cite{morganDialogicReadingPotential2008, klimmtEffectanceControlDeterminants2007a}. 

%\begin{quote}
   % AGENT: \textbf{[The Protagonist]} \textit{Now, let's come up with a cool main character for the story. This could be an animal, a person, a mythical creature, or anything else that fits our story. What do you want our main character to be?} 

    %CHILD: \textit{The main character is a panda!}

    %AGENT: \textbf{[The Protagonist's Name]} \textit{That's interesting! What's the character's name?} 

    %CHILD: \textit{Her name is Lucy.}
    
    %AGENT: \textbf{[The Story Setting]} \textit{Great! Where will our story happen?} 

   % CHILD: \textit{It will happen in a forest.}
    
    %AGENT: \textit{Alrignt! We'll dive into an incredible adventure with a panda named Lucy in the forest. Ready to start the story? Let's go!} 
%\end{quote}

% \subsubsection{Story co-creation}
%The agent then generates a story opening tailored to the given elements.

%\begin{quote}
   % AGENT: \textit{Once upon a time, in the heart of a lush green forest, lived a playful panda named Lucy. One sunny afternoon, she found an unusual map, and along with her new friend, a little child named Nick (the child's avatar), they embarked on an exciting journey to find a hidden treasure.}
%\end{quote}

%From there, Alexa asks the child an open-ended question, listens to the response, and creates content based on that response. 

%Depending on how the child responds, Alexa either provides positive feedback and continues the story, asks a follow-up question for clarity such as, ``\textit{What a good point! Who should we ask for help? Can you tell me more about these helpful friends?}'', or provides ideas if the child's response does not contain usable content (i.e. says "I don't know" or remains silent)~\cite{lamottBirdBirdInstructions1995, zhangStoryDrawerChildAI2022,zhangStoryDrawerCoCreativeAgent2021,sunCollaborativeStorytellingRobot2017}. 
%This technique is widely utilized in conversational agents~\cite{graesserAutoTutor2012,graesserIntelligentTutoringSystems2012}.

%\begin{quote}
    %AGENT: \textit{What will Lucy and Nick do next to make sure the sum of their steps equals the total distance to the treasure?}
    
    %CHILD: \textit{I don't know.}
    
    %AGENT: \textbf{[Hint and Rephrase Scaffolding]} \textit{That's okay! Let's think together. Lucy and Nick can take turns counting their steps. If they keep track, how can they make sure their total steps equal the distance to the treasure?}
%\end{quote}

%If the child still did not provide content, the agent simply continued the story and asked a new question. After six iterative rounds of co-creation, the agent concludes by summarizing the story. This recapitulation serves to consolidate the child's learning and reinforce information retention~\cite{bernardEffectsRecapStrategies1985}.



%\begin{quote}
  %  AGENT: \textbf{[Co-creative Storytelling]} \textit{Lucy and Nick decided to seek the wise counsel of Lucy's father, Mr. Bamboo. He examined the map and told them, ``The treasure is hidden a \textbf{sum} total of 100 steps away from the ancTje ient oak tree.'' He then added, ``You must also find the half-way point, which is \textbf{half} of the total steps, that is, 50 steps from the start.''}
    
  %  AGENT: \textbf{[In-Context Math Word Explanation]} \textit{In this context, ``\textbf{sum}'' means all together, like 100 steps total, and ``\textbf{half}'' is when you split something into two equal parts, like 50 steps.}
    
   % AGENT: \textbf{[Real-time Question Generation]} \textit{How will Lucy and Nick use the \textbf{sum} of steps and the \textbf{half}-way point to find the treasure?}
    
    % \textit{Question: How will Lucy and Nick use the \textbf{sum} of steps and the \textbf{half}-way point to find the treasure?}

  %  CHILD: \textit{Lucy goes to the halfway point; I go to the end, and finally we find all the treasure!}

   % AGENT: \textbf{[On-the-Fly Feedback]} \textit{Wonderful idea! That's a clever way to divide and conquer the search.}
%\end{quote}

%The narrative adheres to the \textit{quest} archetype, a widely prevalent plot in children's literature~\cite{huckChildrenLiteratureElementary2003}. This entails a storyline centered on the protagonist's pursuit of a specific location, object, or objective, overcoming numerous challenges in the process. To enhance children's engagement, their avatar is designed as the protagonist's partner throughout the adventure.

% The five key design goals (DG), as detailed below, were based on the research literature highlighted in the previous section.

% \begin{enumerate}

% \item[\textbf{DG1}]
% \label{DG1} 
% \textbf{Teaching Mathematical language through Exposure and Practice.}
% The mathematical terms taught in our system were selected based on those frequently utilized in state and national mathematical knowledge standards, such as the Common Core State Standards~\cite{councilofchiefstateschoolofficersCommonCoreState2010}.
% However, given that the complete pool of terms is too extensive to cover at once, we focus on six representative terms—\ie \textit{sum}, \textit{estimate}, \textit{add}, \textit{subtract}, \textit{equal}, \textit{half}—to demonstrate our system's capabilities.
% As exposure and practice are critical in language skill development~\cite{kungRoleMathematicalLanguage2019,purpuraCausalConnectionsMathematical2017,sonParentalMathTalk2020}, our system aims to provide children with repeated opportunities to be exposed to and practice using these mathematical vocabulary terms.

% \item[\textbf{DG2}]
% \label{DG2}
% \textbf{Tailoring Story Content Diversity to Children's Preferences.}
% Previous storytelling-based interventions, like dialogic reading, depend on predefined storybooks and planned questions~\cite{purpuraDevelopmentMathematicalLanguage2019,purpuraEngagingCaregiversChildren2021}.
% This approach can lead to the exhaustion of available materials and potentially cause children to lose interest after repeated readings~\cite{biemillerEffectiveMethodBuilding2006}.
% As children often feel more engaged when they perceive a sense of autonomy and competency in their storytelling~\cite{ryanMotivationalPullVideo2006}, our goal is to empower them to personalize story elements (\eg protagonist) and shape storylines. 
% Subsequently, the system automatically generates story content tailored to their preferences.

% \item[\textbf{DG3}]
% \label{DG3}
% \textbf{Co-Creating Stories by Adaptively Integrating Children's Contributions.} 
% Prior research demonstrates that the collaboration between children and AI can alleviate cognitive challenges in story creation, inspire creativity, and encourage more active verbal engagement~\cite{zhangStoryDrawerChildAI2022,zhangStoryDrawerCoCreativeAgent2021,sunCollaborativeStorytellingRobot2017}.
% An essential aspect of such collaboration is acknowledging and integrating contributions from both parties during the creative process, ensuring that AI feedback adapts to the child's input.
% Therefore, our goal is to design a system that can flexibly incorporate children's responses into feedback and seamlessly continue the story based on children's additions.

% \item[\textbf{DG4}]
% \label{DG4}
% \textbf{Encouraging Children's Active Participation through Creativity Support.}
% During the co-creative storytelling process, it's crucial that children actively participate rather than merely listen passively~\cite{morganDialogicReadingPotential2008}.
% Moreover, children may sometimes struggle to progress the story, reaching impasses where they cannot envision the next step~\cite{zhangStoryDrawerChildAI2022,lamottBirdBirdInstructions1995}.
% To address this, we aim to use the question-feedback-scaffolding framework~\cite{xuElinorTalkingMe2022}, , generating immediate prompts (\ie questions, acknowledgements, hints) to stimulate thoughtful responses from children, foster positive engagement, and kindle their creativity.
% \end{enumerate}

% \begin{figure*}
% \centering
% \includegraphics[width=\linewidth]{figures/user_flow.jpg}
% \caption{The interaction flow of the \TOOL system.}
% \Description{}
% \label{user_flow}
% \end{figure*} 


% \begin{figure*}
% \centering
% \includegraphics[width=\linewidth]{figures/implementation.jpg}
% \caption{Technical pipeline of the \TOOL system illustrated with a conversation example. Each feature utilizes an independent GPT module.}
% \Description{}
% \label{implementation}
% \end{figure*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/all-in-one.jpg}
\caption{The interaction flow of the \TOOL system.}
\Description{}
\label{fig:all_in_one}
\end{figure*} 

%\subsection{User Flow}
%The agent initiates the interaction by introducing itself as ``Alexa'', inquiring about the child's name and asking how the child feels. This warning up is intended to put the child at ease, as such a social exchange is familiar to them and the question is one they can answer with confidence. Then, to promote the child's active involvement in story creation processes, the agent solicits their input for key narrative elements like deciding on the protagonist and setting~\cite{morganDialogicReadingPotential2008, klimmtEffectanceControlDeterminants2007a}. Following this, Alexa and the child collaboratively embark on the storytelling journey:  The agent first generates a story opening tailored to the given elements. In the opening, the child's avatar is portrayed as the protagonist's partner to enhance their engagement. From there, Alexa asks the child an open-ended question, listens to the response, and creates content based on that response. After six iterative rounds of co-creation, the agent concludes by summarizing the story. The example conversation between a child and the agent can be found in Appendix~\ref{sec:example_conversation}.\looseness=-1 
% This recapitulation serves to consolidate the child's learning and reinforce information retention~\cite{bernardEffectsRecapStrategies1985}.


\subsection{Prompt Engineering}
The model underlying \TOOL was GPT-4\footnote{\url{https://openai.com/gpt-4}}, currently the most advanced LLM available for developers. Through prompt engineering, GPT-4 performed two primary tasks: 1) generating questions to facilitate children's continuation of the story; and 2) continuing the story based on children's responses, including in-context explanations of math terms. In addition, GPT-4 was used to categorize the type of support that children might require for effective engagement in story co-creation and subsequently generated scaffolding or follow-up questions. The prompts were developed through an iterative process. We borrowed Brown et al.~\cite{brownLanguageModelsAre2020a} suggested prompt engineering strategies to draft our initial draft. We then underwent a two-month-long revision process, which involved internal evaluations with the research team and evaluations with children, and this process led us to rapid iterations of the prompts.

%to extract story elements from the user's responses, evaluate whether the user effectively continues the story, and generate encouraging and scaffolding responses, as shown in Fig.~\ref{implementation}. 
All these features were implemented using the OpenAI APIs\footnote{\url{https://platform.openai.com/docs/api-reference/chat}}.
The final version of prompts used in the user study is displayed in Appendix~\ref{sec:appendix_prompt} Table~\ref{tab:prompt_list}.
% We combined a rule-based method and a LLM-based intent classification method to identify whether the user successfully continues the story, offers a very short response or fails to extend the story.
% Firstly, the LLM-based classifier determines whether the given text expresses a feeling or emotion in the first person, such as uncertainty, agreement, satisfaction, or interest, such as ``\textit{I don't know}'', ``\textit{I'm not sure}'', and ``\textit{Please go on}''.
% If yes, we prompted 
% The rule-based method will calculate the number of words in the user's response.

% This information is discussed further in the following sections.

\subsubsection{Question Generation}

%LLMs support in-context few-shot learning via prompting—instead of finetuning or re-training models for each new task, one can prompt an LLM with a few input and output data exemplars from the target task.
%Previous work has demonstrated that this few-shot prompting performs competitively with benchmark approaches for many language processing tasks such as question generation~\cite{brownLanguageModelsAre2020a}. Our model evaluation, detailed in the following section, reaffirmed these findings.

Following a similar prompt structure proposed in Brown et al.'s work~\cite{brownLanguageModelsAre2020a}, each prompt starts with a preamble which explains the prompt's purpose: ``\textit{Given an unfinished story, compose one single, straightforward question to prompt a 6-year-old to expand on the story.}''
The preamble is followed by a detailed list of instructions and multiple exemplars consisting of the input and the output. Specifically, we directed the model to pose questions concerning the main character's subsequent actions or emotions. These two story elements are not only important to the narrative's progression but are also tangible concepts that children can readily engage with and respond to ~\cite{paris2003assessing}. To enhance GPT-4 performance, we provided six exemplar questions generated by the research team. These questions were further reviewed and approved by two trained research assistants in the domains of children's verbal storytelling and mathematics education. 
The detailed prompt templates are shown in Appendix~\ref{sec:appendix_prompt} Table~\ref{tab:prompt_list}.

\subsubsection{Story Continuation} 
To facilitate the continuation of stories based on children's inputs, while integrating mathematical language instruction, we began by prompting the model to assume the role of a "\textit{storytelling robot}". This prompt established the interactive framework of the LLM's responses.

The next part of the prompt was focused on context-setting. We supplied the model with a narrative scenario: ``\textit{Let's play a joint storytelling game where we build a story together with the main character being a [character] named [name] in the [setting].}'' The elements in brackets ([character], [name], [setting]) would be dynamically populated based on the responses provided by the children. 

For the model to produce coherent and math-focused responses, we articulated a specific sequence for it to follow. The model was tasked with acknowledging children's contributions, utilizing a minimum of two mathematical terms, and then offering in-context explanations. This was achieved via the following detailed prompt:
``\textit{First, acknowledge my addition and commend me in a concise 10-word sentence. Next, continue the story by correctly using [mathematical term one] and [mathematical term two] or their variants within two distinct 15-word sentences. Lastly, explain their meanings within a 20-word sentence, grounding it firmly within the story's context.}''

During experimentation, we observed the LLM's tendency to occasionally overlook prior directives as interactions continued. To counter this behavior and maintain consistency, our specific instructions were reiterated with each turn. This ensured \TOOL's alignment with our intended conversational flow.

% Additionally, a moderation layer was integrated to analyze the content generated by the model, using the OpenAI APIs\footnote{\url{https://platform.openai.com/docs/api-reference/moderations}}, to ensure it contained no instances of sexual content, hate speech, harassment, violence, or self-harm.
%This was in preparation for subsequent prompts that would be combined with the children's responses. 
%\hl{The model is instructed to recognize the child's input, and expand on the story utilizing at least two mathematical terms (or their variants), while explaining their meanings within the story's context. Word limits were imposed to maintain brevity and avoid redundancy.}


\subsection{Model Evaluation}
As part of the iterative design process, we conducted an evaluation to examine the technical capabilities of our LLM-powered system. Specifically, our goal was to confirm whether the prompt-engineered GPT-4 model performs satisfactorily and whether its performance surpasses that of a fine-tuned GPT-3.5 model. This evaluation consisted of two components: firstly, assessing the model's ability to \textit{generate questions} to elicit children's responses to determine if these questions are fluent, inspirational, and logically relevant; secondly, evaluating the model's performance in \textit{generating and continuing stories} that are both logically relevant and engaging. All evaluations were carried out by three college student research assistants who had over a year of experience in educational research and extensive years of engagement in activities with children within the target age range of our study. These students underwent training until their inter-rater reliability reached a satisfactory level before beginning the actual evaluation.

\subsubsection{Evaluating Prompt Engineered GPT-4's Performance in Question Generation}

The generated questions are designed to inspire children to continue the story and encourage them to learn and use mathematical terms. In this evaluation, we compared our prompt-engineered GPT-4 model with a fine-tuned GPT-3 model. The fine-tuned GPT-3 model was trained\footnote{\url{https://platform.openai.com/docs/guides/fine-tuning}} using a subset of 100 out of 300 human-crafted questions developed by an author of the paper. Besides these two LLMs, we also included the other subset of human-crafted questions as our baseline.

The question evaluation included four matrices, namely \textit{readability}, \textit{inspiration}, \textit{story relevancy}, and \textit{math language relevancy}. We invited the three evaluators to score the questions across each of the four dimensions in a 5-point Likert scale. The inter-rater reliability among these evaluators was satisfactory with an average of intra-class correlation of 0.82 across four dimensions. Details of these matrices are presented in Table~\ref{tab:expert_evaluation_question}.

\begin{table*}
\small
\centering
\caption{Metrics and measuring questions used in evaluating prompt engineered GPT-4's performance in question generation. The average intraclass correlation coefficient (\textit{ICC}) scores are displayed.}
\label{tab:expert_evaluation_question}
\begin{tabularx}{1.06\textwidth}{lXl}
\toprule
\textbf{Metric} & \textbf{Description} & \textbf{\textit{ICC}}\\
\hline
Readability & The generated question is written in understandable English, using proper grammar and vocabulary. & 0.758 \\
Inspiration & The generated question stimulates children's thinking and provokes them to articulate their thoughts. & 0.870 \\
Story Relevancy & The generated question aligns with the narrative plotline. & 0.751\\
Math Language Relevancy & The generated question requires children's understanding or use of specific mathematical terms. & 0.907\\
\bottomrule
\end{tabularx}
\end{table*}


\begin{table*}
\small
\centering
\caption{The statistical metrics of the results of the question generation evaluation, where the ANOVA test p-values (*: \textit{p}<.05, **: \textit{p}<.01, ***: \textit{p}<.001) are reported.}
\label{tab:question_generation}
\begin{tabular}{llccccccccl}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Factor}}} & 
\multicolumn{2}{c}{Human} & 
\multicolumn{2}{c}{Fine-tuned GPT-3} & 
\multicolumn{2}{c}{Prompted GPT-4} & 
\multicolumn{3}{c}{Statistics} \\ 
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
\cmidrule(lr){8-8}
\cmidrule(lr){9-9}
\cmidrule(lr){10-10}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\textit{M}} & 
\multicolumn{1}{c}{\textit{SD}} & 
\multicolumn{1}{c}{\textit{M}} & 
\multicolumn{1}{c}{\textit{SD}} & 
\multicolumn{1}{c}{\textit{M}} & 
\multicolumn{1}{c}{\textit{SD}} & 
\multicolumn{1}{c}{\textit{F}} & 
\multicolumn{1}{c}{\textit{p}} & 
\multicolumn{1}{c}{\textit{sig}} 
\\ 
\toprule
Readability & 4.904 & 0.228 & 4.693 & 0.746 & 4.957 & 0.139 & 9.415 & $<$.001 & *** \\ 
Inspiration & 4.571 & 0.532 & 4.281 & 0.892 & 4.713 & 0.467 & 11.357 & $<$.001 & *** \\ 
Story Relevancy & 4.700 & 0.401 & 4.327 & 0.839 & 4.779 & 0.392 & 17.327 & $<$.001 & *** \\
Math Language Relevancy & 2.987 & 0.710 & 1.607 & 0.921 & 2.911 & 0.811 & 90.687 & $<$.001 & *** \\
\bottomrule
\end{tabular}
\end{table*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/question_generation.jpg}
\caption{The distribution of data and the results from the ANOVA post-hoc Tukey's HSD test regarding the question generation evaluation. Statistically significant results are reported as \(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\). Error bars represent 95\% confidence intervals (CIs).}
\Description{}
\label{fig:question_generation}
\end{figure*}

An ANOVA was conducted to compare the ratings of questions generated by human, fine-tuned GPT-3, and our prompt-engineered GPT-4 model. The results indicated significant differences among the sources for all four dimensions (Table~\ref{tab:question_generation}).
A post hoc Tukey's HSD test further revealed that questions generated by both humans and GPT-4 exhibited higher levels of readability, inspiration, and relevance to the story's plot and mathematical language when compared to questions generated by the fine-tuned GPT-3 model (Figure~\ref{fig:question_generation}). The evaluation ratings between human-generated and GPT-4 generated questions were comparable, further suggesting the feasibility and promise of GPT-4 models in this context. \looseness=-1


\subsubsection{Evaluating Prompt Engineered GPT-4's Performance in Story Continuation}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/story_preference.jpg}
\caption{The evaluation results on three metrics of story continuation.}
\Description{}
\label{fig:story_preference}
\end{figure*}

\TOOL is designed to continue the story adaptively based on children's contributions and integrate mathematical language within the story plot. To evaluate whether our prompt-engineered GPT-4 model achieved these two goals, we compared the GPT-4 generated stories with those generated by humans as our baseline, given that other existing models were not tailored to continue stories but rather generate new stories. GPT-4 generated stories were created using a self-chat technique ~\cite{ghandehariounApproximatingInteractiveHuman2019}, which enabled our dialogue system to engage in self-generated conversations, mimicking a child's interactions, and collaboratively creating stories. Human-generated stories were based on the same instructions we provided to prompt GPT-4. The data set crafting process is detailed in Appendix~\ref{sec:appendix_dataset}. Subsequently, we presented the three evaluators with pairs of stories, one generated by GPT-4 and the other by humans. We asked them to make a choice or indicate a tie from each pair based on four dimensions: \textit{preference}, \textit{perceived creativity}, and \textit{mathematics relevancy}, using a widely recognized method for evaluating AI-generated dialogues~\cite{liACUTEEVALImprovedDialogue2019}. Table ~\ref{tab:expert_evaluation_story} provides a detailed explanation of these metrics.


\begin{table*}
\small
\centering
\caption{Metrics and measuring questions used in evaluating prompt engineered GPT-4's performance in story continuation.}
\label{tab:expert_evaluation_story}
\begin{tabular}{ll}
\toprule
\textbf{Metric} & \textbf{Question}\\
\hline
Preference & Who would you prefer to collaborate with to create a story? \\
Perceived Creativity & Whose story sounds more creative and contains more twists and turns?\\
Mathematics Relevancy & Whose story contains more mathematical elements?\\
\bottomrule
\end{tabular}
\end{table*}

The results of this evaluation are displayed in Fig~\ref{fig:story_preference}. Overall, our evaluators indicated that over half of the story pairs, where one was generated by humans and the other by GPT-4, were comparable in quality across all dimensions. However, the evaluators showed a slight preference for human-generated stories and perceived them as more creative than those generated by GPT-4. In contrast, evaluators noted that GPT-4-generated stories excelled in incorporating mathematical language and elements when compared to human-generated stories. Based on discussions with our evaluators, it became evident that one of GPT-4's shortcomings in terms of creativity lies in its tendency to produce storylines that, while coherent, can be somewhat monotonous. These narratives often focus on a single scene or action without branching out into other elements. On the other hand, GPT-4's advantages in relating stories to mathematical elements are likely due to the fact that this task capitalizes on LLMs' capabilities of creating seemingly logical connections of language elements based on specific instructions. 


%From this, we compiled a collection of 8 conversations, each consisting of six dialogue rounds, forming a complete story.
%Then, we recruited two graduate students in education to create another 8 stories via six rounds of human-to-human dialogue.
%We provided these human narrators with a detailed list of specific instructions like the list of mathematical terms they have to use.
%The story content told by one speaker during each dialogue round is deemed a story continuation. 
%In total, we compiled 96 LLM-crafted and 96 human-crafted story continuations for our evaluation. 






\subsection{System Implementation}
\TOOL is a desktop application designed to run on a MacBook computer with built-in microphones and speakers. 
This application, written in Python, does not rely on any graphical interface for interaction. 
Instead, users can navigate \TOOL simply by voice. 
Upon launch, users have the flexibility to specify both the number of dialogue rounds and the mathematical terms they wish to learn. 
For voice-based interaction, \TOOL leverages the Google Cloud Speech-to-Text API\footnote{\url{https://cloud.google.com/speech-to-text}} to recognize users' verbal inputs. 
Additionally, the Elevenlabs Speech Synthesis service\footnote{\url{https://beta.elevenlabs.io/speech-synthesis}} is employed to generate realistic speech for the agent's responses.

% \TOOL runs on a Macbook computer with a built-in microphone and speakers.
% It is not dependent on any graphical interface to interact with and can be navigated simply by voice.
% When launching \TOOL, the users can determine the number of dialogue rounds and the mathematical terms to be learned.

% \TOOL is a desktop application written in Python.
% To realize voice-based interaction, we utilized the Google Cloud Speech-to-Text API\footnote{\url{https://cloud.google.com/speech-to-text}} for recognizing the child's saying and employed the Elevenlabs Speech Synthesis service\footnote{\url{https://beta.elevenlabs.io/speech-synthesis}} to generate a realistic speech for the agent's responses.


% \subsection{Development Process}
% We developed \TOOL through an iterative process...

==> sections/4-expert-evaluation.tex <==
\section{Human Evaluation}
\label{sec:expert_evaluation}
% We evaluated \TOOL through a expert evaluation and a user study (Section~\ref{sec:user_study}).
The human evaluation was conducted to demonstrate the technical capabilities of our LLM-empowered system in co-creative storytelling interactions.

% \TODO{We focused on evaluating these two modules since they are core features and ...}
\hl{Each was compensated with a voucher worth USD $50$.}

% \subsection{Participants}

\subsection{Story Continuation}

% {
% \small
% \begin{xltabular}[h]{\linewidth}{lX}
%     \caption{\TODO{Measuring questions used in our expert evaluation to measure the story style preferences.}} \label{tab:expert_evaluation_story}\\
    
%     \toprule
%     \textbf{Metric} & \textbf{Question}\\ 
%     \midrule
%     \endfirsthead
    
%     \multicolumn{2}{r}{continued from the previous page}\\
%     \toprule
%     \textbf{Metric} & \textbf{Question}\\ 
%     \endhead

%     \multicolumn{2}{r}{to be continued}\\
%     \endfoot
    
%     \hline
%     \endlastfoot
%     Engagingness & Who would you prefer to collaborate with for a long story? \\
%     Interestingness & If you had to say one of these storytellers is interesting and one is boring, who would you say is more interesting? \\
%     Humanness & Which storyteller sounds more human?\\
%     Knowledgeable & If you had to say that one speaker is more knowledgeable and one is more ignorant, who is more knowledgeable?\\
% \bottomrule
% \end{xltabular}
% }
\subsubsection{Experimental Setup}
The purpose of story continuation is to adaptively integrate users' contributions and expose the users to mathematical language through engaging story content.
Thus, guided by prior studies~\cite{leeCoAuthorDesigningHumanAI2022,leeInteractiveChildrenStory2022,liACUTEEVALImprovedDialogue2019,nicholsCollaborativeStorytellingLargescale2020}, we evaluated the research assistants' acceptability of the story continuation and their perceptions of story style.
As the story continuation task in this paper differs from general story generation, it is unfair to compare our LLM-based method with any other existing story generation models.
Therefore, we set human-crafted content as the baseline.
We adopted the self-chat technique as proposed by Ghandeharioun et al.~\cite{ghandehariounApproximatingInteractiveHuman2019}, allowing our dialogue system to interact with itself. 
From this, we compiled a collection of 8 conversations, each consisting of six dialogue rounds, forming a complete story.
Then, we recruited two graduate students in education to create another 8 stories via six rounds of human-to-human dialogue.
We provided these human narrators with a detailed list of specific instructions like the list of mathematical terms they have to use.
\hl{This storytelling task took around 420 minutes and we paid them USD $80$ for their time.}
The story content told by one speaker during each dialogue round is deemed a story continuation. 
In total, we compiled 96 LLM-crafted and 96 human-crafted story continuations for our evaluation. 
% (\TODO{see XX in the Supplementary Materials}).

\paragraph{\textbf{Story Continuation Acceptability}}
Inspired by Lee et al.'s work~\cite{leeCoAuthorDesigningHumanAI2022} that measured how helpful LLM generations are to writers, we annotated the acceptability of candidate story continuations by asking the three trained research assistants to classify each continuation as either \textit{acceptable} or \textit{unacceptable} given the context of the story generated so far.
In order to circumvent potential discrepancies, we resorted to majority voting among the three assigned labels to determine the final label. 
The continuation performance was subsequently calculated using the following metric: \textsc{the number of accepted continuations} / \textsc{the number of total continuations}.

\paragraph{\textbf{Story Style Preferences}}
Following the ACUTE-EVAL method~\cite{liACUTEEVALImprovedDialogue2019} which is widely used for evaluating generated dialogues, we presented trained research assistants with two conversations side by side: one from our LLM-based method and one from the human narrators.
The research assistants were also provided with four measurement questions (Table~\ref{tab:expert_evaluation_story}) and were asked to make a choice between the two conversations or to choose \textit{tie} for each question.
We collected three sets of research assistants' judgments for each comparison pair, using majority voting to determine whether our LLM-based method outperformed the human narrative, or if the result was a \textit{tie} (i.e., a majority opting for \textit{tie}).
We created our own evaluation metric informed by the attributes targeted by ACUTE-EVAL (Table~\ref{tab:expert_evaluation_story}), namely, \textit{Engagingness}, \textit{Interestingness}, \textit{Creativity}, and \textit{Mathematics}, and adapted the optimizing questions to accommodate our specific contexts of joint storytelling and mathematical language, similar to~\cite{nicholsCollaborativeStorytellingLargescale2020}. 
Moreover, we encouraged research assistants to provide their own reasoning for each judgment to gain deeper insights. 
In total, we evaluated 64 paired comparisons.

\subsubsection{Results}


% \begin{figure*}
% \centering
% \includegraphics[width=0.9\linewidth]{figures/story_preference.jpg}
% \caption{Overall expert evaluation results for the four metrics of story style preferences.}
% \Description{}
% \label{fig:story_preference}
% \end{figure*}

\begin{table*}
\small
\centering
\caption{Human evaluation results on four metrics show. For each measurement question, the percentage of researchers that preferred our system's story continuations, the human's contributions, or chose that it was a tie. The chi-square test compared whether GPT-4 or humans significantly outperformed the other across the four dimensions, excluding ties (\(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\)).}
\label{tab:expert_evaluation_story_results}
\begin{tabular}{lcccc}
\toprule
& \textbf{Engagingness} & \textbf{Interestingness} & \textbf{Creativity} & \textbf{Mathematics}\\
\hline
\textbf{GPT-4} & 15.63\% (10) & 12.50\% (8) & 15.63\% (10) & 23.44\% (15) \\
\textbf{Human} & 28.13\% (18) & 37.50\% (24) & 31.25\% (20) & 00.00\% (0) \\
\textbf{Tie} & 56.25\% (36) & 50.00\% (32) & 53.13\% (34) & 76.56\% (49) \\
\hline
\(\chi^2\) test & \(\chi^2(1) = 2.286, p = .131\) & \(\chi^2(1) = 8.0, p = .004^{**}\) & \(\chi^2(1) = 3.333, p = .067\) & \(\chi^2(1) = 15.0, p < .001^{***}\) \\
\bottomrule
\end{tabular}
\end{table*}

We first evaluated the acceptability of story continuations. 
The results showed that 100\% of human-crafted and 97.92\% of LLM-crafted story continuations are acceptable. 
A chi-squared test indicated that there is no significant difference between them (\(\chi^2(1) = 0.502, p = .477\)).
The unacceptable LLM-crafted story continuations were due to (1) the introduction of a previously unmentioned character or (2) repeating previous content without advancing the storyline.
For instance, in the sentence ``\textit{Samantha decided to include the wise old owl's advice in her journey plan.}'', the character ``\textit{the wise old owl}'' appears abruptly, having never been mentioned previously in the story.

In terms of storytelling style preferences, as shown in Table~\ref{tab:expert_evaluation_story_results}, the results suggest that our method and human storytellers are closely matched; they tie in over 50\% of the cases across all four dimensions. 
Delving deeper, and excluding ties, we utilized a chi-square test for further insights (Table~\ref{tab:expert_evaluation_story_results}). 
The test results highlighted that in terms of \textit{Engagingness} and \textit{Creativity}, there is no significant difference between our method and human performance. 
This implies that our method is capable of delivering engaging and creative storytelling experiences on par with humans.
However, when it comes to \textit{Interestingness}, humans outperform our method. 
A plausible reason, as per the raters' explanations, is that our method tends to produce storylines that are somewhat homogenous, often concentrating on a singular theme. 
In contrast, for the dimension of \textit{Mathematics}, our approach surpasses human storytellers. 
This superior performance can be attributed to our method's aptitude to seamlessly integrate in-context explanations of terms within the narrative. 
In comparison, human storytellers occasionally revert to providing only the original definition of terms.\looseness=-1
% Overall, our method showcases promise in certain dimensions of storytelling, achieving comparable performance to humans in areas like engagingness and creativity. 
% While there is room for improvement in diversifying storylines for enhanced interestingness, the method's proficiency in contextual explanations for mathematical terms sets it apart.

\subsection{Question Generation}
\subsubsection{Experimental Setup}
The generated questions are designed to inspire children to continue the story and encourage them to learn and use the mathematical terms.
They are open-ended and relate to what will happen in the story.
However, the state-of-the-art question generation models are targeted to generate question-answer pairs for existing storybooks.
The questions generated by these models are related to what has happened in the story and not sensitive to mathematical language.
Therefore, in this evaluation task, we still set human-crafted content as one of the baselines.
In addition, since OpenAI allows developers to fine-tune the GPT-3 model to enhance its ability to complete a specific generative task in one single dialogue\footnote{\url{https://platform.openai.com/docs/guides/fine-tuning}}, we set the fine-tuned GPT-3 as another baseline.
To craft a dataset, we invited two graduate students in education to create questions for 210 story continuations generated by the above LLM-based method.
\hl{This question writing task took around 300 minutes and we paid them USD $60$ for their time.}
Then, we randomly sampled 100 (as suggested by OpenAI guides) human-crafted questions as a training set to fine-tune GPT-3, while the remaining will be the human baseline.\looseness=-1

\paragraph{\textbf{Generated Question Perceptions}}
Based on the literature~\cite{leeInteractiveChildrenStory2022,yaoItAITurn2022a}, we invited trained research assistants to score the questions across four dimensions in a 5-point Likert scale by giving the associated story content: \textit{Readability}, \textit{Inspiration}, \textit{Question-Story Relevancy}, and \textit{Question-Mathematical Language Relevancy}. 
The detailed descriptions of these dimensions are shown in Table~\ref{tab:expert_evaluation_question}.
The whole list of candidates consists of 110 questions generated by each of our prompted GPT-4 model, the fine-tuned GPT-3 model, and the human, for a total of 330.
When shown to researchers, these questions were randomized and concealed with condition labels.
The researchers first sampled 10\% questions, scored independently, and then discussed to conclude a consensus scoring rubric.
Afterward, they continued to score the remaining samples.
We finally obtained the average intraclass correlation coefficient (\textit{ICC}) scores of 0.758 (\textit{Readability}), 0.870 (\textit{Inspiration}), 0.751 (\textit{Question-Story Relevancy}), and 0.907 (\textit{Question-Mathematical Language Relevancy}).\looseness=-1

\subsubsection{Results}

\begin{table*}
\small
\centering
\caption{Metrics and measuring questions used in the human evaluation to measure the quality of generated questions. ML refers to Mathematical Language.}
\label{tab:expert_evaluation_question}
\begin{tabularx}{\textwidth}{lX}
\toprule
\textbf{Metric} & \textbf{Description}\\
\hline
Readability & The generated question is in readable English grammar and words. \\
Inspiration & How the generated question is inspirational for children to create. \\
Question-Story Relevancy & How the generated question is relevant to the story.\\
Question-ML Relevancy & How answering the question requires children to understand or use specific mathematical terms.\\
\bottomrule
\end{tabularx}
\end{table*}

% \begin{table*}
% \small
% \centering
% \caption{The statistical metrics of the expert evaluation for the question generation, where the ANOVA test p-values (*: \textit{p}<.05, **: \textit{p}<.01, ***: \textit{p}<.001) are reported.}
% \label{tab:question_generation}
% \begin{tabular}{llccccccccl}
% \toprule
% \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Factor}}} & 
% \multicolumn{2}{c}{Human} & 
% \multicolumn{2}{c}{Fine-tuned GPT-3} & 
% \multicolumn{2}{c}{Prompted GPT-4} & 
% \multicolumn{3}{c}{Statistics} \\ 
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-3}
% \cmidrule(lr){4-4}
% \cmidrule(lr){5-5}
% \cmidrule(lr){6-6}
% \cmidrule(lr){7-7}
% \cmidrule(lr){8-8}
% \cmidrule(lr){9-9}
% \cmidrule(lr){10-10}
% \multicolumn{1}{c}{} & 
% \multicolumn{1}{c}{\textit{M}} & 
% \multicolumn{1}{c}{\textit{SD}} & 
% \multicolumn{1}{c}{\textit{M}} & 
% \multicolumn{1}{c}{\textit{SD}} & 
% \multicolumn{1}{c}{\textit{M}} & 
% \multicolumn{1}{c}{\textit{SD}} & 
% \multicolumn{1}{c}{\textit{F}} & 
% \multicolumn{1}{c}{\textit{p}} & 
% \multicolumn{1}{c}{\textit{sig}} 
% \\ 
% \toprule
% Readability & 4.904 & 0.228 & 4.693 & 0.746 & 4.957 & 0.139 & 9.415 & $<$.001 & *** \\ 
% Inspiration & 4.571 & 0.532 & 4.281 & 0.892 & 4.713 & 0.467 & 11.357 & $<$.001 & *** \\ 
% Question-Story Relevancy & 4.700 & 0.401 & 4.327 & 0.839 & 4.779 & 0.392 & 17.327 & $<$.001 & *** \\
% Question-ML Relevancy & 2.987 & 0.710 & 1.607 & 0.921 & 2.911 & 0.811 & 90.687 & $<$.001 & *** \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/question_generation.jpg}
\caption{The distribution of data and the results from the ANOVA post-hoc Tukey's HSD test regarding the human evaluation of question generation. Statistically significant results are reported as \(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\). Error bars represent 95\% confidence intervals (CIs).}
\Description{}
\label{fig:question_generation}
\end{figure*}

An ANOVA was conducted to compare the researchers' ratings of questions generated by a human, fine-tuned GPT-3, and our method (\ie prompted GPT-4) across the four dimensions.
The results indicated significant differences among the sources for all dimensions (Figure~\ref{fig:question_generation}).
A post hoc Tukey's HSD test was performed to further explore these differences. 
The results revealed that questions generated by humans and our method received significantly higher ratings across all the dimensions compared to those by fine-tuned GPT-3 (Figure~\ref{fig:question_generation}). 
Our method performed best across \textit{Readability}, \textit{Inspiration}, and \textit{Question-Story Relevancy}, with average ratings of 4.957, 4.713, and 4.779, respectively.
However, no significant differences were found between the scores for humans and our method.
This indicates that our method can effectively emulate human-like quality in question generation, demonstrating its feasibility in our co-creative storytelling task to prompt children by questioning.\looseness=-1

==> sections/5-user-study.tex <==
\section{User Study}
\label{sec:user_study}
To understand how \TOOL might support children's engagement and math language learning, we conducted a user study where children were randomly assigned to either co-create stories with \TOOL or with a friendly and skilled human partner. We examined children's gains in mathematical language knowledge, their engagement and enjoyment in the story co-creation activities, and the patterns of the stories that emerged from this interaction.


% Moreover, we compared the on-the-fly performance of AI and human interventionists in terms of story continuation (\textit{\textbf{RQ4}}) and question generation (\textit{\textbf{RQ5}}).

\subsection{Procedure}
Participants were recruited from two public libraries in a mid-west city in the U.S. throughout the summer of 2023. This study was approved by the Institutional Review Board of the authors' institution. After obtaining parental consent and child assent, participants were introduced to a research assistant and began the three-part study procedure which consisted of a baseline assessment, the story co-creation activity, and a learning evaluation. All parts of the procedure were recorded on Zoom for later transcription of the stories and coding of open-ended questions. Participants had the option of completing all three parts in a single session or completing the baseline assessment one day and returning another day to complete the story creation activity and learning evaluation. While children were completing the story creation activity, parents were provided with a questionnaire on an iPad to collect demographic information about their child. Once the child completed the procedure they were given a small prize and a book as a thank you and parents received a twenty-dollar Visa gift card for their participation.

\paragraph{\textbf{Baseline}}
% We began by evaluating children's baseline theory of mind attribution to machines, animals, and natural artifacts (i.e. robot, cheetah, mountain). 
% Then we assess children's knowledge of the six mathematical vocabulary target words (add, subtract, equal, estimate, half, sum).
We began by assessing children's knowledge of the six mathematical vocabulary target words (\textit{add}, \textit{subtract}, \textit{equal}, \textit{estimate}, \textit{half}, \textit{sum}).
First, we read the terms out loud to the child and asked the child to repeat the terms. Then, children's knowledge was evaluated using four types of questions: definition, recall, transfer, and practice questions. These are described in more detail in Section~\ref{sec:evaluation_metrics}.\looseness=-1

\paragraph{\textbf{Story Creation Activity}}


\begin{figure*}
\centering
\includegraphics[width=0.4\linewidth]{figures/study_setting.jpg}
\caption{The (a) plushy and (b) speaker used in our user study.}
\Description{}
\label{fig:study_setting}
\end{figure*}

Children were randomly assigned to the human or AI condition to determine their partner for the story creation activity. 
Children were handed a plushy (Figure~\ref{fig:study_setting}(a)) in case they wished to act out the story or just hold on to it. 
During the activity, children co-created two stories.
Each story was approximately seven minutes long. 
One research assistant conducted all the human condition trials and used a physical checklist to keep track of when the words were defined and used per story. 
In the AI condition, children were introduced to the AI as ``my friend,'' which was presented as the Wonderboom 3 speaker by Ultimate Ears (Figure~\ref{fig:study_setting}(b)). 
The researcher then completed a short demo consisting of three exchanges with Alexa to demonstrate how to play the story creation activity. 
Each turn demonstrated the different ways children could interact. 
For the first demo turn the researcher gave a substantive answer, for the second they said ``\textit{I don't know},'' and for the third, they remained silent. 
Then children were free to interact with Alexa without interference or minimal redirection and instructions from the researcher. 
For both \TOOL and human conditions, the story activities typically lasted 6 minutes, with a total of approximately 12 minutes for each child.\looseness=-1
% During the storytelling session the researcher adjusted the input volume as necessary to signal the AI that the child had finished speaking as the hard wear was unable to differentiate when the child had stopped talking due to the background noise in the environment.

\paragraph{\textbf{Learning Evaluation}}
After the story activity children were asked a series of questions about their experience by a second researcher if they had been in the human condition or the same researcher who had facilitated the AI interaction if they had been in the AI condition. 
Then children were asked the same math vocabulary questions from the baseline assessment using different nouns for the transfer set of questions (i.e. ``\textit{you have a jar filled with candies}'' was changed to ``\textit{you have a net filled with butterflies}''). 
This was to ensure children were not merely replicating their answers from the baseline condition. \looseness=-1

\subsection{Participants}

\begin{table*}
\small
\centering
\caption{Participant information by study conditions.}
\label{tab:participant_information}
\begin{tabularx}{0.9\textwidth}{lcccc}
\toprule
 & \textbf{Full Sample} & \textbf{AI} & \textbf{Human} & \textbf{Difference}\\
\hline
Mathematical Language Baseline & 16.686 & 17.105 & 16.188 & \(T(33) = 0.279, p = .391\) \\
Age & 6.000 & 6.105 & 5.875 & \(T(33) = 0.497, p = .623\) \\
Female & 54.29\% (\(N = 19\)) & 52.63\% (\(N = 10\)) & 56.25\% (\(N = 9\)) & \(\chi^2(1) = 0.046, p = .830\) \\
% \textit{Age} & & & & \(\chi^2(4) = 1.900, p = .754\) \\
% \ \ \ \ \ 4-year-olds & 20.00\% (\(N = 7\)) & 21.05\% (\(N = 4\)) & 18.75\% (\(N = 3\)) & \\
% \ \ \ \ \ 5-year-olds & 17.14\% (\(N = 6\)) & 10.53\% (\(N = 2\)) & 25.00\% (\(N = 4\)) & \\
% \ \ \ \ \ 6-year-olds & 17.14\% (\(N = 6\)) & 18.75\% (\(N = 3\)) & 18.75\% (\(N = 3\)) & \\
% \ \ \ \ \ 7-year-olds & 34.29\% (\(N = 12\)) & 42.11\% (\(N = 8\)) & 21.05\% (\(N = 4\)) & \\
% % \ \ \ \ \ 8-year-olds & 11.43\% (\(N = 4\)) & 10.53\% (\(N = 2\)) & 12.50\% (\(N = 2\)) & \\
\textit{Race/Ethnicity} & & & & \(\chi^2(4) = 4.500, p = .343\) \\
% \ \ \ \ \ Asia & 14.29\% (\(N = 5\)) & 10.53\% (\(N = 2\)) & 20.00\% (\(N = 3\)) & \\
\ \ \ \ \ Black & 11.43\% (\(N = 4\)) & 15.79\% (\(N = 3\)) & 6.25\% (\(N = 1\)) & \\
\ \ \ \ \ Latino & 8.57\% (\(N = 3\)) & 5.26\% (\(N = 1\)) & 12.50\% (\(N = 2\)) & \\
\ \ \ \ \ White & 60.00\% (\(N = 21\)) & 68.42\% (\(N = 13\)) & 50.00\% (\(N = 8\)) & \\
\ \ \ \ \ Others & 17.14\% (\(N = 6\)) & 10.53\% (\(N = 2\)) & 31.25\% (\(N = 5\)) & \\
% \textit{Predominant Home Language} & & & & \\
% \ \ \ \ \ English & & & & \\
% \ \ \ \ \ Other & & & & \\
\textit{Parents' Education} & & & & \(\chi^2(2) = 3.240, p = .198\) \\
\ \ \ \ \ Above Bachelor's degree & 34.29\% (\(N = 12\)) & 47.37\% (\(N = 9\)) & 20.00\% (\(N = 3\)) & \\
\ \ \ \ \ Bachelor's degree & 54.29\% (\(N = 19\)) & 42.11\% (\(N = 8\)) & 68.75\% (\(N = 11\)) & \\
\ \ \ \ \ Less than Bachelor's degree & 11.43\% (\(N = 4\)) & 
10.53\% (\(N = 2\)) & 12.50\% (\(N = 2\)) & \\
% \textit{Family Income} & & & & \\
% \ \ \ \ \ Below \$20,000 & & & & \\
% \ \ \ \ \ From \$20,000 -- \$39,999 & & & & \\
% \ \ \ \ \ From \$40,000 -- \$59,999 & & & & \\
% \ \ \ \ \ From \$60,000 -- \$79,999 & & & & \\
% \ \ \ \ \ From \$80,000 --\$99,999 & & & & \\
% \ \ \ \ \ From \$100,000 -- \$149,999 & & & & \\
% \ \ \ \ \ From \$150,000 + & & & & \\
% \ \ \ \ \ Prefer not to say & & & & \\
\textit{Usage of CA} & & & & \(\chi^2(4) = 1.689, p = .793\) \\
\ \ \ \ \ Daily & 17.14\% (\(N = 6\)) & 21.05\% (\(N = 4\)) & 12.50\% (\(N = 2\)) & \\
\ \ \ \ \ Weekly & 17.14\% (\(N = 6\)) & 21.05\% (\(N = 4\)) & 12.50\% (\(N = 2\)) & \\

\ \ \ \ \ Monthly & 14.29\% (\(N = 5\)) & 15.79\% (\(N = 3\)) & 12.50\% (\(N = 2\)) & \\
\ \ \ \ \ Less than once a month & 28.57\% (\(N = 10\)) & 21.05\% (\(N = 4\)) & 37.50\% (\(N = 6\)) & \\
\ \ \ \ \ Never & 22.86\% (\(N = 8\)) & 21.05\% (\(N = 4\)) & 25.00\% (\(N = 4\)) & \\
\hline
\ \ \ \ \ N & 35 & 19 & 16 & \\
\bottomrule
\end{tabularx}
\end{table*}

We recruited 35 participants (19 female, 16 male) aged between four and eight (\(mean = 6\), \(std = 1.35\)) by advertising on online platforms such as Twitter, Reddit, and various college online communities and through snowball sampling. 
% Prior to the study, we evaluated the children's mathematical language skills (Section~\ref{sec:math_language_assessment}) to establish a baseline and control for variables. 
Participants were randomly allocated to either the experimental condition using our system (\(n = 19\)) or the control condition involving a human partner (\(n = 16\)). 
All the participants' predominant home language is English.
No significant differences were observed between the two conditions in terms of gender, age, mathematical language skills, race/ethnicity, prior use of conversational agents, or caregiver education (Table~\ref{tab:participant_information}).

% \subsection{Interventionists}
% Three graduate students implemented the intervention in the control condition.

\subsection{Evaluation Metrics}
\label{sec:evaluation_metrics}
We developed a new questionnaire to assess the mathematical learning outcomes and drew on prior research to evaluate their story creation performance.
Then, we analyzed the children's responses to quantify their engagement and used an established questionnaire to measure their enjoyment.
% Furthermore, we employed the same evaluation techniques used in Section~\ref{sec:expert_evaluation} to assess the real-time performance of both AI and human interventionists in story continuation and question generation.
In this section, we introduce the metrics and analysis process.

\subsubsection{Mathematical Language}
\label{sec:math_language_assessment}
To assess children's learning through the interactions, a 24-item questionnaire was developed based on the Common Core State Standards~\cite{akkus2016common} and Purpura et al.'s work~\cite{purpuraNonlinearRelationsApproximate2015}. It aimed to measure children's grasp of six specific terms (i.e., \textit{sum}, \textit{estimate}, \textit{add}, \textit{subtract}, \textit{equal}, \textit{half}) across four facets: \textit{definition}, \textit{recall}, \textit{transfer}, and \textit{practice}. 
Each facet comprised six questions, one for each term. 
All items were structured to not necessitate exact quantitative skills like counting or calculating.
The complete questionnaire can be found in Appendix~
\ref{sec:appendix_math}.\looseness=-1

For the \textit{definition} dimension, children were prompted to provide the definition of each of the six math terms. In the \textit{recall} dimension, they were asked to identify each term when its definition was given. For \textit{transfer} questions, children needed to provide an appropriate math term based on a provided real-life scenario. Lastly, in the \textit{practice} dimension, children were asked to use the target math terms to describe a picture featuring various fruits.

The \textit{definition} and \textit{practice} items were open-ended and rated either 0 (incorrect) or 1 (correct). 
With \textit{recall} and \textit{transfer} items, children initially attempted to answer without assistance.
If unsuccessful, they were presented with three options. A score of 2 was given for unprompted correct answers, a score of 1 for correct answers with given prompts, and a score of 0 for incorrect answers.
Based on this scoring system, we calculated a total score by summing the points across all items, with a possible range from 0 to 36. 
The Cronbach's alpha of the learning outcome items was 0.92.

\subsubsection{Story Creation Performance}
We analyzed the number of ideas and elaborations from 1) children's responses to AI or human storytellers, and 2) story continuations by the AI or human, to evaluate their storytelling performance. 
Based on prior work~\cite{wongSpokenNarrativeAssessment2016,zhangStoryDrawerChildAI2022},
% Idea fluency is represented by the number of creative ideas in narratives.
a creative idea is defined by a character and its associated action within a single utterance. 
For instance, ``\textit{The cat climbs the tree}'' presents one idea, with ``\textit{cat}'' as the character and ``\textit{climbs}'' as its associated action. 
% Idea elaboration, on the other hand, is denoted by the extent of detail added in the narratives.
An elaboration pertains to the supplementary details (\eg when, where, why) introduced after presenting a creative idea. 
For example, ``\textit{The bird sings beautifully at dawn because it's mating season}'' provides details about the timing and reason, thereby earning two points.
One coded the transcripts for all participants, while the other coded 30\% of the participants as a quality check, yielding \textit{ICC} of over 0.85.
\looseness=-1

\subsubsection{Engagement}
To quantify children's verbal engagement, we evaluated six items from the children’s responses during the co-creative storytelling activities.
First, we calculated the average number of words in each child's response.
Next, we determined whether a child verbally responded to the prompt, marking this as the response rate.
If a response was given, we coded and calculated the percentage of: meta-comments that describe the child's thought process (\eg ``\textit{I like it.}''), uncertainty responses (\eg ``\textit{I don't know.}''), short responses (fewer than 5 words), and substantial responses.
This coding was carried out by two trained research assistants.
One coded the transcripts for all participants, while the other coded 30\% of the data as a quality check. 
The agreement rate between these two coders was 100\% across all items.\looseness=-1

\subsubsection{Enjoyment}
To measure children's enjoyment when interacting with AI or humans, we adapted a 4-item questionnaire from Waytz et al.'s work~\cite{waytzMindMachineAnthropomorphism2014}. Each item is rated on a 5-point Likert scale, ranging from 1 (no) to 5 (absolutely), and was presented immediately after the story creation activity. The questions include: 
(1) \textit{Did you enjoy your story reading session with []?}; 
(2) \textit{Did you feel comfortable reading with []?}; 
(3) \textit{Would you like to have a reading partner like []?}; and 
(4) \textit{Do you want to read another story with []?}.
The calculated Cronbach's alpha is approximately 0.77.

\subsection{Results}

\subsubsection{Mathematical Language}
As shown in Figure~\ref{fig:mathematical_language}, we first employed a paired t-test to compare pre-post-test scores in each condition. In the experimental condition using our system, there were significant improvements across three dimensions: \textit{definition}, \textit{transfer}, and \textit{practice}.
A significant improvement was also observed in the total score (\(T(18) = -3.520, p = .002^{**}\)).
However, our system did not facilitate significant gains in \textit{recall}.
In the control condition with a human partner, significant improvements were observed in \textit{transfer},  \textit{practice}, and the total score (\(T(15) = -3.032, p = .008^{**}\)).
However, the human partner did not significantly enhance participants' gains in \textit{definition} and \textit{recall}.
We conducted an independent t-test to compare improvements between the two conditions. 
No significant differences were identified in \textit{recall}, \textit{transfer}, \textit{practice}, and the total score (\(T(33) = -0.104, p = .541\)).
However, there was a significant difference in \textit{definition}.
Children demonstrated greater gains in understanding mathematical term meanings when using our system as compared to human intervention.
In sum, our system achieved comparable performance to human intervention in enhancing children's transfer and practice abilities in mathematical language.
Our system also surpassed human intervention in bolstering their understanding of terms but both the human partner and the system were not effective in enhancing recall. This may be a result of recall questions requiring a working memory of the six terms.\looseness=-1

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/mathematical_language.jpg}
\caption{Box plots showing the data distribution and the results of the paired t-test for the pre-post-test within each condition, as well as the results of the independent t-test comparing the two conditions in terms of improvements in the mathematical language assessment. Statistically significant results are reported as \(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\).}
\Description{}
\label{fig:mathematical_language}
\end{figure*}

\subsubsection{Story Creation Performance}

\begin{figure*}
\centering
\includegraphics[width=0.6\linewidth]{figures/story_creation_performance.jpg}
\caption{Box plots illustrating the data distribution, along with the results of the independent t-test, comparing two conditions for the story creation performance of children, and AI v.s. humans. Statistically significant results are reported as \(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\).}
\Description{}
\label{fig:creation_performance}
\end{figure*}

We initially conducted an independent t-test to assess the differences in children's story creation performance between the AI and human conditions. 
As depicted in Figure~\ref{fig:creation_performance}(a), there is no marked distinction in terms of the number of ideas (AI: \(M = 0.443, SD = 0.392\), Human: \(M = 0.616, SD = 0.404\)) or elaborations (AI: \(M = 0.285, SD = 0.336\), Human: \(M = 0.360, SD = 0.390\)) of children across both conditions.
This suggests that our system offers a level of support to children's story creation process that is on par with human assistance. 
We also contrasted the creation performances of AI and the human partner (Figure~\ref{fig:creation_performance}(b)).
Notably, while the number of ideas generated by the AI and human partner did not significantly differ, the AI produced considerably more detailed elaborations (\(M = 2.585, SD = 0.417\)) compared to humans (\(M = 1.938, SD = 0.983\)).
A closer look at Figure~\ref{fig:creation_performance}(b) reveals that our system's performance is more consistent than the human partner, as evidenced by the narrower interquartile range.\looseness=-1 

% elaborations & ideas -> narrative patterns
While the number of elaborations and ideas is easily quantified, the quality of the ideas and elaborations is harder to analyze. The AI often elaborated on already present elements of the story, adding ideas that enhanced emotion or scenery, whereas the human elaborated on elements not yet present adding ideas that advance the plot. See examples in Table~\ref{tab:human_ai_story}. This distinct pattern created a recursive narrative structure in the AI condition and a divergent narrative structure in the human condition. 

\begin{table}[H]
\small
\centering
\caption{Comparative example scenarios of children providing short responses during interactions with \TOOL and humans.}
\label{tab:human_ai_story}
\begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}b{6cm}|>{\raggedright\arraybackslash}b{\dimexpr\linewidth-6.5cm-2\tabcolsep\relax}}
\toprule
\textbf{\textsc{Mathmyths}} & \textbf{Human}\\
\hline
\textit{``Using his mighty wings, Scaly added included flight to their adventure. Lifting off the ground, the sum total of their happiness was as vast as the endless sky above them.''}& \textit{``They proceeded due north towards what they expected to be the destination of the magical tree. When they were halfway there, so when they were an equal part into the woods, and an equal part left in the woods, they discovered that there was a big log in the middle of the road.''}\\
\hline
\textit{``Their faces lit up equally with joy as they discovered the treasure. The joy they felt was equal to the amount of effort they had put in the journey.''}& \textit{``Finally, they arrived in Virginia. They got off the plane, and then they realized that they didn't know where the brother lived. Luckily they brought the seashell.''}\\
\bottomrule
\end{tabularx}
\end{table}

\begin{table}[H]
\small
\centering
\caption{The statistical metrics of children's verbal engagement in each condition, where the independent t-test p-values (\(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\)) are reported.}
\label{tab:engagement}
\begin{tabular}{lccccccl}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Engagement}}} & \multicolumn{2}{c}{AI} & \multicolumn{2}{c}{Human} & \multicolumn{3}{c}{Statistics} \\ \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-8}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textit{M}} & \multicolumn{1}{c}{\textit{SD}} & \multicolumn{1}{c}{\textit{M}} & \multicolumn{1}{c}{\textit{SD}} & \multicolumn{1}{c}{\textit{T}} & \multicolumn{1}{c}{\textit{p}} & \multicolumn{1}{c}{\textit{sig}} \\ 
\toprule
Average Length & 6.806 & 5.297 & 9.750 & 6.108 & \(-\)2.160 & 0.034 & * \\ 
Response Rate (\%) & 93.721 & 11.604 & 98.229 & 4.739 & \(-\)2.056 & 0.044 & * \\
Response Category & & & & & & & \\
\ \ \ \ \ \textit{Meta Comments Rate (\%)} & 9.771 & 13.033 & 5.861 & 6.179 & 1.555 & 0.125 & --- \\
\ \ \ \ \ \textit{Uncertainty Response Rate (\%)} & 9.913 & 15.539 & 1.842 & 5.708 & 2.782 & 0.007 & ** \\
\ \ \ \ \ \textit{Short Response Rate (\%)} & 40.757 & 19.987 & 36.586 & 18.791 & 0.894 & 0.375 & --- \\
\ \ \ \ \ \textit{Substantial Response Rate (\%)} & 33.280 & 30.833 & 53.941 & 23.459 & \(-\)3.107 & 0.003 & ** \\
\bottomrule
\end{tabular}
\end{table}

Figure~\ref{fig:narrative_structure} provides examples. In the AI narrative, the plot points are repeatedly about a giraffe attempting to reduce its mass but never sufficiently reducing its size. In this case, the child introduced the only movement in the narrative by introducing a crack that the house was falling into, but the narrative turned once again to the giraffe attempting to reduce its mass. By contrast, in the human narrative, the plot points move the characters closer to the goal of finding a book and conclude with the characters successfully finding the book.

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/narrative_structure.jpg}
\caption{Comparative narrative structure crafted by \TOOL and humans: Notably, (a) the AI demonstrates a recursive pattern, while (b) humans exhibit a divergent structure.}
\Description{}
\label{fig:narrative_structure}
\end{figure*}


% \hl{A few examples in Table~\ref{tab:human_ai_story} show a common pattern in AI elaboration.} 

% second difference:  details whether it is peripheral or central/ 
% find examples of AI's pointless descriptions and human's on-point descriptions 2 for each 

% \textsc{Mathmyths}: \textit{Using his mighty wings, Scaly added included flight to their adventure. Lifting off the ground, the sum total of their happiness was as vast as the endless sky above them}.

% \textsc{Mathmyths}: \textit{Their faces lit up equally with joy as they discovered the treasure. The joy they felt was equal to the amount of effort they had put in the journey}. 

% Human: \textit{They proceeded due north towards what they expected to be the destination of the magical tree. When they were halfway there, so when they were an equal part into the woods, and an equal part left in the woods, they discovered that there was a big log in the middle of the road}.

% Human: \textit{Finally, they arrived in Virginia. They got off the plane, and then they realized that they didn't know where the brother lived. Luckily they brought the seashell}. 



% Lastly, when averaging out the story creation performance to evaluate whole stories, collaborations between children and AI remain statistically indistinguishable from those between children and human interventionists.
In conclusion, while there were some interesting qualitative differences, our system was more consistent than the human partner
which highlights its potential as a reliable creative collaborator for children.\looseness=-1

\subsubsection{Engagement}
We conducted an independent t-test to compare the AI condition with the human condition in terms of children's verbal engagement.
As shown in Table~\ref{tab:engagement}, children verbally responded to over 90\% of the questions in both conditions, which means they engaged with both the AI and human partner during the storytelling activity. There was no significant difference in terms of the rate of meta-comments or the rate of short responses. In both conditions, over 35\% of children's responses were fewer than five words, aligning with previous research on interactive dialogic reading~\cite{xuElinorTalkingMe2022}.
However, how children engaged was significantly different depending on their interaction partner.
In the human partner condition, the rate of children's uncertainty responses was significantly lower and the rate of children's substantial responses was significantly higher than with the AI partner. 

The number of uncertain responses in the AI condition could be attributed in part to the unusual problems the AI asked the child to solve. For example: AI asked, ``\textit{How do you think they will estimate the distance remaining, and use the cloud to add speed to their journey?}'', while the child responded, ``\textit{I don't know.}''
Not only does this require children to understand what "estimate" means by this point in the story, but the question is very difficult to answer. How could a cloud be used to increase speed? By contrast, the human partner provided children with opportunities to problem-solve that were more grounded in children's real-life experience of the world. For instance, the human partner may asked, ``\textit{How do you think they should take away some cars so they can get through the traffic circle?}'', and the child answered: ``\textit{Take away seventeen cars and then just drive off.}'' 
A possible explanation for the insignificant difference in short responses is likely because short answers were often sufficient to answer questions posed by both the AI and human partner as shown in Table~\ref{tab:human_ai_short_response}.
In sum up, children are more engaged and responsive when interacting with humans than AI.\looseness=-1

\begin{table}[H]
\small
\centering
\caption{Comparative example scenarios when children give a short response when interacting with \TOOL and humans.}
\label{tab:human_ai_short_response}
\begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}b{9.5cm}|>{\raggedright\arraybackslash}b{\dimexpr\linewidth-10cm-2\tabcolsep\relax}}
\toprule
\textbf{\textsc{Mathmyths}} & \textbf{Human}\\
\hline
AI: \textit{``What do you think they could make together?''} 
\newline Child: \textit{``Pie.''} & Human: \textit{``What food should they bring?''}
\newline Child: \textit{``umm Chicken nuggets.''}\\
\hline
AI: \textit{``How do you think Zombie will add or subtract pebbles to continue the game?''}
\newline Child: \textit{``Finding more?''} & Human: \textit{``How big is the friend?''}
\newline Child: \textit{``Up to Chungy's belly.''}\\
\bottomrule
\end{tabularx}
\end{table}

% AI: What do you think they could make together? 
% Child: Pie

% AI: How do you think Zombie will add or subtract pebbles to continue the game?
% Child: Finding more?

% Human: What food should they bring?
% Child: umm Chicken nuggets

% Human: How big is the friend?
% Child: Up to Chungy's belly.
% This is in line with our expectations, as we observed that human interventionists (\(M = 22.156, SD = 11.377\)) were more responsive and used continuous back-and-forth to elicit significantly more responses from children (\(T(68) = -4.386, p < .001^{***}\)) than AI (\(M = 13.921, SD = 2.032\)), which was designed to further prompt children in up to two rounds.

% Third point substantial responses: difference 
% AI: resposne to the question; Human: continuaing the response; moving the plot 

% turn-taking pattern; interjection here


\subsubsection{Enjoyment}

We conducted an independent t-test to assess children's enjoyment between the two conditions. 
As shown in Figure~\ref{fig:enjoyment}, it appeared that children showed a slightly higher preference for the human storyteller, but the difference is not significant. Overall, children enjoyed the story co-creation activity, but did not want to read another story with either partner. 

One explanation for this seemingly confusing result is that the baseline questions had already taken up a significant portion of the children's patience and the storytelling task, while fun, was also mentally taxing. We had a few children declare that they needed a nap during or shortly after the storytelling activity. In one case, we allowed a child to nap on the table for ``5 minutes'' which actually turned out to be 30 seconds in order to finish the study. Another possible contribution to children's preference might stem from the occasional errors the AI made in recognizing children's words, resulting from the limitations of the Speech-to-Text API we utilized. Finally, children's tendency to prefer a human partner might simply be due to interfacing with a simple speaker in the AI condition and a physically present human in the human condition. Children's increased enjoyment in the human condition may be directly related to extra social feedback they received from interacting with a live person and may not necessarily be related to the differences in story co-creation. \looseness=-1

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/enjoyment.jpg}
\caption{The distribution of data and the results from the independent t test regarding children's enjoyment. Statistically significant results are reported as \(p < 0.05^{*}\), \(p < 0.01^{**}\), \(p < 0.001^{***}\). Error bars represent 95\% confidence intervals (CIs).}
\Description{}
\label{fig:enjoyment}
\end{figure*}

% \subsubsection{On-the-fly Question Generation \& Story Continuation}

\subsubsection{Turn-Taking Pattern}
A general consideration for these results is children's propensity to interrupt the human partner. This often was a result of perceived eagerness to continue the story or correct the human partner if the child decided they wanted the narrative to go a different direction. This kind of frequent interjection was not seen in the AI condition, likely because it became apparent to children that their interjections were ignored. These interruptions may have impacted a number of the findings above. For example, it may have impacted math learning outcomes because these interruptions sometimes happened during the definitions part of the human partner turn. For example:

Human: \textit{Yes, the bones snapped in half which means half it was equal to--}.

Child: \textit{this but it was like was like had to make it's like this. Then it was like that and then it was like}.

Human: \textit{yes. And so then they made a cast that was equal to the size of her ear--}.

Child: \textit{They didn't use a cast. They used bandaid}.

Human: \textit{They used a bandaid--}

Child: \textit{But they used this big up of bandaid. They put an ear bandaid on like that so they could show she}.

Human: \textit{so the bandaid was equal size of her ear--}.

Child: \textit{Then sister got to grab her, then they went home. And now your turn to add}.

Next, the human partner had fewer elaborations and ideas likely in part because children were providing them as seen in the higher frequency of substantial responses (Table~\ref{tab:engagement}). The more substantial responses a child gave, the less the human partner needed to provide these elements. Finally, children's tendency to interrupt and interject with their own ideas counter to those provided by the human partner points to a level of enjoyment and ownership over the activity not seen in the explicit measures. In sum, the human partner's ability to listen and respond to, or inability to ignore and continue on in the face of, interjection may have significant consequences for the way children learn, create stories, engage, and enjoy this approach for learning math vocabulary. 

==> sections/6-discussion.tex <==
\section{Discussion}
This paper offers an exploration into the potential of using LLMs to craft conversational systems for teaching mathematical language via child-AI co-creative storytelling. Our iterative design and development process provides insights into how prompt engineering methods might feasibly be adapted to suit LLMs for young children in a specific educational context, and the model evaluation suggests that prompt-engineered LLMs could produce questions and stories approaching human-like quality. A subsequent user study further showed that the math learning outcomes were also comparable, yet the patterns of children's engagement and the narrative structures of the co-created stories differed. 

In the remainder of this section, we will discuss how our study speaks to the growing body of literature on child-AI interactions and how we introduce new evidence to still under-explored areas, the use of LLMs as conversational partners. We will then discuss design implications that could guide future developments. Finally, we will address potential limitations and outline a future research agenda. 

\subsection{Leveraging LLMs for Educational Tools}
The capability of LLMs has attracted much attention from researchers to build educational tools for children~\cite{kasneciChatGPTGoodOpportunities2023}.
Following this trend, this paper explored how to optimize LLMs as story co-creators for children's mathematical language learning through prompt engineering. 
During our development, we noted that LLMs, due to their broad generative capabilities, can be less predictable than specialized machine learning models crafted for distinct tasks. The primary reason is that the nuances of how LLMs interpret our prompts remain a ``black-box'' for developers. 
In our efforts at prompt-engineering, there was no guarantee that revising prompts would consistently yield the desired outcomes. This unpredictability aligns with findings in recent literature~\cite{duanShiftingAttentionRelevance2023,linGeneratingConfidenceUncertainty2023}. To create a prompt that consistently produces intended results, multiple iterations, coupled with trial and error, were necessary. However, refining prompts is relatively quick, especially compared to traditional AI model fine-tuning or training. %In other words, while there may be more iterations, each one is relatively short in duration. 

%Addressing it required us to perform more iterations. However, each iteration was swift due to the sole refinement of prompts, potentially making the development faster than conventional methods. Yet, it is worth noting that while iterations are faster, their number might increase because of the need to understand LLMs' interpretation nuances based on prompts. 
%Striking the right balance between prompt generality and desired output specificity is vital for optimal performance.

While LLMs' impressive general language capability allows for easy instruction based on descriptive language, it remains a challenge to provide precise directives to control the output specifically. A significant aspect of this challenge is associated with LLM's limited capacities in numerical reasoning~\cite{zhangLargeLanguageModels2023}. For instance, given that \TOOL was tailored for young children, we aimed to use brief and simple language to facilitate comprehension. However, when we set specific word limits within each sentence for GPT-4 (e.g., ``\textit{each sentence should not exceed 10 words}''), the model often disregarded such constraints. In contrast, descriptive instructions without numeric values, like ``\textit{keep language brief and child-friendly},'' consistently produced better results. In light of these limitations, other research recommends incorporating mechanisms for quality checks when precision in output is a priority. Feedback loops~\cite{leeReliableFluentLarge2023} and validation layers~\cite{he-yueyaSolvingMathWord2023} have been suggested to ensure the model's output aligns with the desired requirements.

A final observation pertains to LLMs occasionally sidestepping structural directives during prolonged interactions~\cite{zhaoSurveyLargeLanguage2023,whitePromptPatternCatalog2023}. As an example, if GPT-4 is directed to maintain a specific narrative structure in its responses, it might stray if these instructions are front-loaded. To counteract this, we employed injection prompting, strategically placing reminders within ongoing interactions. By doing so, we enhanced response consistency and adherence to the desired structural format.\looseness=-1

% LLMs iterative, higher degree of uncentainty 
% require more iteration, yet each iteration is quick 

% sensitivity to numbers 

% remind


% \subsection{Child-AI Co-Creative Storytelling for Mathematical Language Learning}
% In general, our system met the design objective of providing children with repeated opportunities to learn mathematical language through exposure and practice.
% Children co-creating stories with our system showed significant improvements in their understanding, transfer, and practice of mathematical terms.
% Although our study was based on two storytelling sessions, sustained interaction with \TOOL over extended periods might lead to enhanced mathematical abilities, considering the causal connections between mathematical language and mathematical knowledge~\cite{purpuraCausalConnectionsMathematical2017,purpuraNonlinearRelationsApproximate2015}.
% In terms of understanding, children interacting with our system surpassed their peers who engaged with trained human partner.
% This might be attributed to \TOOL's capability to generate in-context explanations for introduced terms, which are intertwined with the storyline, making them more conducive to children's comprehension.
% Despite their training, human partner sometimes failed to provide such in-context explanations on-the-fly.

% Our study also provided initial evidence of the benefits of child-AI co-creative storytelling on children's creativity.
% While there were no differences in children's performance between interactions with AI or humans, the AI's output was more consistent than that of human partner and even included significantly more story details.
% This consistency might foster the long-term development of creativity in children, as prior studies suggest children can learn or emulate creativity from AI partners~\cite{aliCanChildrenEmulate2020,aliCanChildrenLearn2019}.

% Furthermore, children enjoyed their interactions with our system, aligning with previous studies on storytelling systems~\cite{zhangStoryBuddyHumanAICollaborative2022,zhangStoryDrawerCoCreativeAgent2021,xuExploringYoungChildren2020}.
% Before our system, past research focused on joint storytelling either through the Wizard-of-Oz method, where experimenters substituted for the agent~\cite{sunCollaborativeStorytellingRobot2017}, or followed a predefined multi-branch narrative structure~\cite{ligthartDesignPatternsInteractive2020}.
% Thus, our system represents the first fully automatic conversational agent offering children a enjoyable joint storytelling experience.

% Although we anticipated that AI would elicit lengthier and more comprehensive responses from children, human partner outperformed our system.
% A follow-up analysis revealed that the human partner engaged in significantly more back-and-forth dialogue to draw out responses from children, compared to the AI, which was designed to prompt children up to two times.
% This responsive back-and-forth is crucial in encouraging children to express their thoughts and feelings more deeply~\cite{bucholzeddCreatingWarmInclusive2009}.
% Our LLM-based system, while adept at continuous dialogue, might lack the intuitive adaptability and emotional nuance inherent in human partner.

% Computers as social actors
\subsection{AI as Storyteller Partners}
In this paper, we found that although the AI and human partner achieved comparable performance in teaching children mathematical language, children still slightly preferred and engaged more when interacting with the human partner.
This observation is reminiscent of the findings of Harry Harlow's seminal experiments~\cite{harlowNatureLove1958} with rhesus monkeys in the 1950s.
Despite the wire monkey mother providing milk, the infant monkeys showed a clear preference for the cloth-covered surrogate that offered tactile comfort. 
In much the same way, our results indicate that while the virtual agent can effectively impart knowledge, engage children, and provide entertaining stories, there remains something that humans offer that fosters higher quality and more substantial engagement. 
Despite similar learning outcomes other research has also found this human preference %and supports the idea that emotional and social nuances of human interaction play a pivotal role in the learning process (unsupported claim)
~\cite{neumann2023preschool}. However, Westlund et al. ~\cite{westlund2015comparison} found a preference for their fluffy social robot over a human interlocutor for a vocabulary learning task.

Future research interested in exploring children's preferences and engagement with technological learning partners could explore the multi-facets of AI physical presence.
For example, combining the latest developments in haptic design for emotional robotic touch~\cite{zhouDemonstratingTactorBotsHaptic2023} could provide a ``cloth-covered'' AI partner, bridging the gap between the precision of AI and the socially stimulating presence of humans. 

%

%Notably, human preference was also observed when the robot was humanoid ~\cite{neumann2023preschool}
%westlund2015comparison robot preference but robot was fluffy
% These advancements could revolutionize how children perceive and engage with AI, potentially leading to a more harmonious coexistence between humans and machines in educational settings.

% there is an old paper about a robot that gives chimps milk and a cuddly chimp that shocks the baby and gives no milk, but the chimp still prefers the cuddly chimp to the one that provides milk. The point being that even if the AI provides the child with interesting stories, more interesting than humans stories, or more information, or is better in any number of ways, children might STILL prefer to interact with a human because we are more "cuddly." If we put this AI into a "cuddily" cut body children might like it a lot more.


\subsection{Design Considerations}
In this section, we discuss some design implications of our study. 
Our team has already begun improvements to our co-creative storytelling system based on the considerations below.

\subsubsection{Generating Adaptive Questions}
During storytelling, \TOOL generates questions to elicit children's responses. 
However, some children found certain questions challenging to answer. 
This was evident from the notably higher rate of uncertainty in their responses to AI-generated questions compared to those posed by human partner.
While we implemented scaffolding features to assist children when they struggle to respond, the AI might not always capture the nuances of a child's emotions and experiences. Specifically, it may not always discern precisely what factors (e.g., language barriers, math knowledge gaps, or unwillingness to participate) caused their struggle. As a result, while the AI provided some scaffolding based on several broad categories, it did not offer more tailored adjustments in response to the unique challenges faced by individual children. One design consideration is to integrate more adaptive algorithms into LLM-based tools that can accurately assess a child's cognitive load based on their responses and adjust the complexity of the questions accordingly.\looseness=-1

% AI is more mentally taxing, more consideration should be taken to scaffold and lower cogntive demand in participating in the story creation. 

\subsubsection{Providing Creativity Support}
Our study revealed the potential benefits of child-AI co-creative storytelling for enhancing children's creativity. 
Although no performance difference was observed between children interacting with AI or humans, AI demonstrated more consistent outputs, often enriched with detailed story elements.
However, we observed that children frequently gestured or moved while speaking, hinting at potential challenges in coming up with stories in an abstract way. 
To address this, future designs could integrate graphical interfaces or multimedia elements, aiding in visualizing their thoughts.
This approach would empower children to externalize their ideas not only through words but also via drawings, animations, and sound effects.
Such externalization have proven to boost children's creativity~\cite{zhangStoryDrawerChildAI2022,zhangStoryDrawerCoCreativeAgent2021} and enhance comprehension of complex concepts like math~\cite{dwivediVisualMathAutomatedVisualization2017}.
In this context, consistent interactions with AI, which might promote long-term creativity in children, become even more significant as they have shown the capability to learn or emulate creativity from AI interactions~\cite{aliCanChildrenEmulate2020,aliCanChildrenLearn2019}.

\subsubsection{Supporting Embodied Interaction}
In this paper, \TOOL utilizes a virtual conversational agent to engage children in joint storytelling. 
While this platform can be easily navigated via voice, it might fall short in conveying emotions or actions---a vital aspect that captivates children during interactions with human counterparts. 
To compromise it during our user study, we provided children with a plushy. 
Nonetheless, this might not fully capture the advantages of tangible interactions. 
A promising solution could be to integrate this virtual agent with an embodied robot, which can offer more vivid feedback through its human-like expressions and behaviors~\cite{hubbardChildRobotInteractionIntegrate2021,whiteDesigningEmotionallyExpressive2021}. 
It is potential that an embodied robot could stimulate different or perhaps heightened levels of engagement.
However, the cost implications and scalability concerns associated with robots cannot be ignored.


% portable; mobile vesrion embodiement although it is possible that an embodied robot would elicit different, or likely higher engagemnet,  robots are expensive, less likely to be scaled up etc. % eventhough we provide a plushie, but it might not be enough. 




% \subsubsection{Supporting Parent-AI Collaboration}

\subsection{Limitations and Future Work}
While our study offers preliminary insights, it also paves the way for addressing further questions in the future. 

First, in our user study, we compared children's interactions with \TOOL with those with a trained researcher who adhered to a strict protocol for narrating stories. This protocol ensured the inclusion of a specified number of mathematical terms. While this approach granted us a controlled environment, ensuring consistent mathematical language exposure for the children, it might have constrained the natural adaptability and spontaneity that a human experimenter can bring to the storytelling process. In future research, it would be intriguing to also compare children's engagement and enjoyment with a human partner who can fully harness their natural storytelling capabilities. Related, we compared the learning outcomes between two storytelling conditions but did not include a comparison to more conventional instructional methods, such as directly teaching the terms, providing examples, allowing the child to practice, and offering corrective feedback.  It remains to be seen whether such a direct and structured approach might offer other benefits over the storytelling conditions in certain contexts or for certain learning objectives.


Second, our study's participants engaged in only two AI collaborative storytelling sessions. This limited exposure might not fully reflect the dynamics of extended interactions children might have with such systems. As children become more accustomed to the AI over time, their expectations could evolve, potentially requiring more advanced and adaptive storytelling experiences. On the other hand, repeated sessions could lead to a more harmonized child-AI collaboration, potentially enriching the storytelling process. Future studies should explore these longer-term dynamics, perhaps by giving children extended opportunities to interact with the AI storytelling system and tracking their engagement patterns over extended periods.


%we utilized a trained human partner as a baseline for comparing our AI system's performance. Both groups followed a set protocol to narrate stories with children and impart mathematical vocabulary. While our AI system demonstrated comparable, if not superior, efficacy in teaching mathematical language, the factors contributing to this success remain ambiguous. Was it the AI's repetitive vocabulary exposure or the interactive story co-creation practice? 


%Firstly, our user study gauged children's immediate mathematical language learning outcomes post-interaction with AI or human partner. This design overlooks children's long-term retention of this language.  To enhance the depth of our findings, subsequent studies could incorporate a delayed post-test and a transfer test, which would more comprehensively evaluate the impact of teaching mathematical language on the development of lasting mathematical skills~\cite{purpuraCausalConnectionsMathematical2017}.

%To discern this, we had intended to introduce a dialogic reading condition~\cite{xuElinorTalkingMe2022}, where the AI narrates a story and poses questions, but does not allow children to shape the narrative.
%Second, although we identified our system achieved performance comparable to human intervention and even better in mathematical language teaching, it is unclear that such benefits were due to the repeated exposure of terms in AI generated stories or the interactive practice of co-creating stories. 
%Indeed, our team had planned to include an additional dialogic reading condition~\cite{xuElinorTalkingMe2022} where the conversational agent told a story and asked children questions but did not allow children to continue the story.
%Third, participants in our study only engaged in a two AI collaborative storytelling sessions. This short engagement may not accurately capture the dynamics of prolonged interactions children might have with such systems. 
%Over time, as the novelty of AI interaction wears off, children's expectations could grow, necessitating a more intricate and responsive storytelling experience. 
%Conversely, recurrent interactions might cultivate a deeper child-AI synergy, fostering enhanced storytelling and creativity. 
%Future research should delve deeper into these longitudinal aspects, possibly by providing children with extended access to the AI storytelling system and observing their interaction patterns over time. Finally, we compared the learning outcomes between two storytelling conditions but did not include a comparison to an explicit conventional method of teaching these math terms. It is possible that the narrative distracted children or provided an additional cognitive load to the task of teaching children mathematical terminology. It could be that a more direct streamlined lesson explicitly teaching, providing examples, and asking the child to practice using the mathematical terms and providing corrective feedback might be a superior method than either storytelling condition. 
% Lastly, there is a burgeoning concern about AI-driven tools becoming integral parts of children's lives, potentially overshadowing human-to-human interactions. 
% We firmly believe that the goal of introducing AI in children's lives should be to complement, not replace, their human interactions, especially in contexts where expert intervention is inaccessible to certain demographics. 
% To bolster parent-child engagements, our future endeavors include designing an AI system to aid parents—lacking formal interventionist training—in collaborative storytelling with their children, especially those of low-SES families.

\subsection{A Note on Ethical Considerations}
The safe use of AI by children has been a topic of public discussion for some time. As we transition to an era dominated by generative AI, the debate becomes even more pressing. In this new landscape, children may directly encounter content produced by AI without the protective filters traditionally provided by human oversight. In this section, we will focus on some ethical considerations pertaining to privacy and safety.

In terms of privacy, \TOOL utilizes two cloud-based services to process children's utterances: Google's speech-to-text for transcribing and OpenAI's GPT-4 to interpret their responses. Both companies offer measures to protect children's data. Specifically, children's utterances are not stored and are promptly deleted after transcription by Google Cloud. Additionally, OpenAI commits not to train their models with data passed through their APIs\footnote{\href{https://openai.com/api-data-privacy}{https://openai.com/api-data-privacy}}. However, when these cloud-based AI products enter the market, the adequacy of children's data privacy protection remains uncertain due to the absence of specific regulations for AI products. While the US Children's Online Privacy Protection Act (COPPA) regulates the collection and use of personal information from those under 13, it has yet to be updated to tackle the emerging concerns related to AI.

In terms of safefy, to safeguard against inappropriate AI-generated content, we integrated a moderation layer, utilizing the OpenAI APIs\footnote{\url{https://platform.openai.com/docs/api-reference/moderations}}, to ensure outputs were devoid of sexual content, hate speech, harassment, violence, or self-harm. However, this content filtering approach might not be as effecgtive in
addressing biases and stereotypes (e.g., when a child asks ``\textit{What do girls do?}'', and the AI agent responds ``\textit{housewives}''), given that these biases are as deeply ingrained in the data used to train AI systems as they are in the rest of the culture. Nonetheless, a growing number of studies have begun to investigate methods for detecting and reducing such stereotypes and biases, although these studies have not specifically focused on children. Given the present state of technology, a viable approach would be to deploy LLMs within a ``walled garden''—limiting interactions to narrower domains, like the math-focused narratives in our study. Such confines might mitigate risks while still capitalizing on the capabilities of LLMs. 

==> sections/7-conclusion.tex <==
\section{Conclusion}

While AI has been utilized for structured interactions with children for quite a while, such as dialogic question-answering, the affordance provided by LLMs in facilitating free-form, creative tasks, like joint storytelling, signifies a groundbreaking shift. This research explores that very frontier. Our findings suggested that, although the learning outcomes with AI mirror those with human partners, the interaction dynamics are different. Instead of viewing this as a limitation, it might be more fruitful to recognize AI as providing a unique interaction opportunity. These interactions, while different, could supplement children's everyday human interactions. Given the rapid advancements in LLMs, the capabilities we observe today are likely to further refine in the near future. Yet, the insights garnered now will shape and anchor our design philosophies as we move forward. \looseness=-1

==> sections/8-acknowledgement.tex <==
\begin{acks}

\end{acks}
